Does progress on ImageNet transfer to real-world datasets?

Does progress on ImageNet transfer to real-world datasets? We investigate this question by evaluating ImageNet pre-trained models with varying accuracy (57% - 83%) on six practical image classification datasets. In particular, we study datasets collected with the goal of solving real-world tasks (e.g., classifying images from camera traps or satellites), as opposed to web-scraped benchmarks collected for comparing models. On multiple datasets, models with higher ImageNet accuracy do not consistently yield performance improvements. For certain tasks, interventions such as data augmentation improve performance even when architectures do not. We hope that future benchmarks will include more diverse datasets to encourage a more comprehensive approach to improving learning algorithms.

==> conclusion.tex <==
\section{Conclusion}


==> future.tex <==
\section{Future work}


==> grids.tex <==
\subsection{CCT-20}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{CCT-20, AlexNet}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04 & 1.00E-05       & 1.00E-06 & 0              \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 29.81    & 29.81    & 29.81          & 29.81    & 29.81          \\
                               & 1.00E-02             & 60.58    & 61.68    & 62.19          & 61.87    & 62.15          \\
                               & 1.00E-03             & 59.43    & 61.74    & 59.55          & 61.57    & \textbf{62.48} \\
                               & 1.00E-04             & 57.82    & 58.25    & 56.76          & 59.34    & 58.99          \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 29.81    & 29.81    & 29.81          & 29.81    & 29.81          \\ 
                               & 1.00E-02             & 57.38    & 58.58    & 59.01          & 60.03    & 58.75          \\
                               & 1.00E-03             & 61.31    & 59.26    & 60.80          & 61.17    & \textbf{62.95} \\
                               & 1.00E-04             & 57.82    & 58.74    & 56.31          & 57.22    & 56.94          \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 29.81    & 29.81    & 29.81          & 29.81    & 29.81          \\
                               & 1.00E-03             & 59.67    & 54.76    & 56.88          & 53.37    & 53.53          \\
                               & 1.00E-04             & 56.05    & 62.29    & \textbf{63.59} & 61.51    & 62.91          \\
                               & 1.00E-05             & 45.61    & 58.48    & 56.62          & 60.03    & 60.24          \\ \bottomrule
\end{tabular}
\end{table}

\begin{table}[h]
\centering
\caption{CCT-20, MobileNet V3 small}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04       & 1.00E-05       & 1.00E-06       & 0     \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 60.42    & 64.44          & 63.82          & 63.47          & 63.59 \\
                               & 1.00E-02             & 64.63    & 63.56          & \textbf{65.32} & 63.85          & 63.99 \\
                               & 1.00E-03             & 62.08    & 62.76          & 62.80          & 60.07          & 60.32 \\
                               & 1.00E-04             & 50.31    & 50.79          & 50.97          & 50.19          & 49.67 \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 64.40    & 64.80          & 64.13          & 64.73          & 64.04 \\
                               & 1.00E-02             & 64.01    & 64.08          & 63.56          & \textbf{64.83} & 63.92 \\
                               & 1.00E-03             & 59.79    & 61.26          & 58.74          & 58.90          & 60.58 \\
                               & 1.00E-04             & 48.36    & 48.93          & 49.34          & 50.08          & 48.60 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 64.65    & \textbf{66.01} & 63.38          & 61.35          & 61.33 \\
                               & 1.00E-03             & 64.75    & 64.05          & 64.74          & 63.39          & 63.21 \\
                               & 1.00E-04             & 53.13    & 62.94          & 62.48          & 62.64          & 63.71 \\
                               & 1.00E-05             & 41.06    & 54.60          & 52.30          & 53.34          & 55.23 \\ \bottomrule 
\end{tabular}
\end{table}


\begin{table}[h]
\centering
\caption{CCT-20, VGG-13 BN}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03       & 1.00E-04 & 1.00E-05 & 1.00E-06       & 0              \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 72.17          & 73.60    & 73.32    & 73.34          & 73.59          \\
                               & 1.00E-02             & 73.76          & 73.12    & 73.66    & 74.08          & \textbf{74.72} \\
                               & 1.00E-03             & 71.71          & 71.34    & 70.86    & 70.52          & 71.42          \\
                               & 1.00E-04             & 61.22          & 60.79    & 60.22    & 61.14          & 60.23          \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 72.24          & 71.57    & 71.56    & 71.92          & 63.72          \\
                               & 1.00E-02             & \textbf{74.53} & 74.00    & 74.14    & 73.62          & 73.49          \\
                               & 1.00E-03             & 71.30          & 70.42    & 70.56    & 71.23          & 70.38          \\
                               & 1.00E-04             & 58.63          & 59.33    & 59.31    & 59.11          & 55.88          \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 29.81          & 45.34    & 40.33    & 29.81          & 43.66          \\
                               & 1.00E-03             & 72.88          & 72.72    & 71.42    & 72.63          & 71.24          \\
                               & 1.00E-04             & 72.79          & 74.69    & 74.02    & \textbf{75.06} & 74.17          \\
                               & 1.00E-05             & 70.22          & 70.93    & 69.78    & 70.38          & 71.08          \\ \bottomrule
\end{tabular}
\end{table}

\begin{table}[h]
\centering
\caption{CCT-20, DeiT-tiny}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04       & 1.00E-05 & 1.00E-06       & 0              \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 40.55    & 31.62          & 38.22    & 31.77          & 35.27          \\
                               & 1.00E-02             & 63.58    & 63.67          & 63.56    & 63.19          & 63.42          \\
                               & 1.00E-03             & 66.56    & 65.70          & 64.76    & \textbf{66.93} & 65.57          \\
                               & 1.00E-04             & 63.48    & 62.00          & 63.00    & 63.70          & 62.08          \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 46.22    & 32.01          & 31.99    & 30.75          & 31.43          \\
                               & 1.00E-02             & 63.73    & 64.85          & 64.39    & 64.17          & 63.34          \\
                               & 1.00E-03             & 65.65    & \textbf{68.77} & 65.63    & 66.87          & 67.28          \\
                               & 1.00E-04             & 60.45    & 60.11          & 60.50    & 61.40          & 59.57          \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 44.34    & 39.93          & 39.20    & 38.99          & 38.81          \\
                               & 1.00E-03             & 48.35    & 51.44          & 54.51    & 50.00          & 50.37          \\
                               & 1.00E-04             & 45.53    & 65.05          & 66.28    & 65.55          & \textbf{66.61} \\
                               & 1.00E-05             & 38.64    & 62.06          & 64.86    & 64.11          & 63.39          \\ \bottomrule
\end{tabular}
\end{table}

\begin{table}[h]
\caption{CCT-20, ResNet-50}
\centering
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03       & 1.00E-04       & 1.00E-05 & 1.00E-06       & 0     \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 47.09          & 46.05          & 47.40    & 49.79          & 46.86 \\
                               & 1.00E-02             & 72.47          & \textbf{72.70} & 70.65    & 71.04          & 70.98 \\
                               & 1.00E-03             & 70.46          & 69.60          & 70.39    & 70.08          & 70.63 \\
                               & 1.00E-04             & 61.29          & 61.45          & 60.87    & 62.00          & 61.00 \\
                                \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 47.83          & 46.28          & 45.07    & 48.65          & 46.93 \\
                               & 1.00E-02             & \textbf{73.96} & 72.51          & 72.49    & 73.34          & 72.46 \\
                               & 1.00E-03             & 69.16          & 70.44          & 70.06    & 70.40          & 70.23 \\
                               & 1.00E-04             & 58.71          & 59.03          & 58.35    & 58.02          & 59.24 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 54.99          & 49.76          & 50.07    & 51.22          & 46.47 \\
                               & 1.00E-03             & 71.22          & 70.86          & 72.19    & \textbf{72.70} & 71.94 \\
                               & 1.00E-04             & 70.30          & 70.38          & 71.27    & 70.98          & 72.38 \\
                               & 1.00E-05             & 68.05          & 68.91          & 69.55    & 69.94          & 69.42 \\ \bottomrule
\end{tabular}
\end{table}


\begin{table}[h]
\centering
\caption{CCT-20, ResNet-152}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04       & 1.00E-05 & 1.00E-06       & 0              \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 47.32    & 46.55          & 50.13    & 48.33          & 49.79          \\
                               & 1.00E-02             & 71.81    & 71.96          & 72.28    & \textbf{73.43} & 73.10          \\
                               & 1.00E-03             & 73.26    & 72.53          & 72.74    & 72.72          & 72.30          \\
                               & 1.00E-04             & 65.12    & 66.26          & 64.90    & 65.99          & 65.29          \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 49.08    & 48.06          & 44.44    & 48.49          & 47.17          \\
                               & 1.00E-02             & 73.99    & \textbf{74.05} & 73.36    & 72.86          & 72.26          \\
                               & 1.00E-03             & 72.70    & 73.29          & 73.26    & 72.21          & 72.95          \\
                               & 1.00E-04             & 62.56    & 63.30          & 63.80    & 62.50          & 63.46          \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 52.30    & 47.72          & 45.55    & 48.72          & 50.94          \\
                               & 1.00E-03             & 70.92    & 69.43          & 69.93    & 71.35          & 70.46          \\
                               & 1.00E-04             & 70.56    & 71.70          & 72.93    & 72.03          & 72.52          \\
                               & 1.00E-05             & 60.79    & 72.14          & 72.18    & 70.87          & \textbf{73.09} \\ \bottomrule 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{CCT-20, DeiT-small}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04       & 1.00E-05 & 1.00E-06       & 0              \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 29.81    & 29.81          & 42.29    & 29.81          & 29.81          \\
                               & 1.00E-02             & 67.68    & 68.43          & 69.06    & 67.24          & 67.46          \\
                               & 1.00E-03             & 70.37    & \textbf{71.41} & 68.96    & 70.75          & 70.46          \\
                               & 1.00E-04             & 63.31    & 62.39          & 63.72    & 62.37          & 61.49          \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 29.98    & 29.35          & 34.52    & 29.50          & 31.49          \\
                               & 1.00E-02             & 68.21    & 67.33          & 68.47    & 68.24          & 68.72          \\
                               & 1.00E-03             & 68.64    & 68.56          & 68.97    & 67.95          & \textbf{69.31} \\
                               & 1.00E-04             & 63.89    & 63.71          & 62.12    & 63.50          & 63.37          \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 46.43    & 37.59          & 38.56    & 37.63          & 35.98          \\
                               & 1.00E-03             & 45.88    & 47.93          & 47.95    & 48.52          & 46.76          \\
                               & 1.00E-04             & 47.42    & 69.46          & 68.75    & \textbf{70.61} & 70.29          \\
                               & 1.00E-05             & 37.85    & 65.40          & 67.31    & 66.22          & 69.08          \\ \bottomrule 
\end{tabular}
\end{table}


\begin{table}[h]
\centering
\caption{CCT-20, PNASNet-5 large}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04 & 1.00E-05       & 1.00E-06 & 0     \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 71.04    & 70.10    & 71.55          & 70.32    & 71.05 \\
                               & 1.00E-02             & 71.78    & 70.75    & \textbf{72.03} & 71.99    & 71.22 \\
                               & 1.00E-03             & 69.60    & 69.08    & 69.31          & 69.37    & 68.31 \\
                               & 1.00E-04             & 59.06    & 59.84    & 59.30          & 60.00    & 58.60 \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 69.42    & 70.98    & 71.51          & 72.78    & 72.11 \\
                               & 1.00E-02             & 72.06    & 72.66    & \textbf{73.41} & 72.07    & 71.86 \\
                               & 1.00E-03             & 68.39    & 68.50    & 67.78          & 68.27    & 68.62 \\
                               & 1.00E-04             & 57.94    & 57.55    & 57.84          & 58.50    & 59.22 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 53.02    & 49.10    & 59.80          & 52.69    & 53.60 \\
                               & 1.00E-03             & 71.24    & 73.05    & \textbf{75.21} & 71.98    & 72.73 \\
                               & 1.00E-04             & 64.63    & 70.90    & 73.03          & 70.06    & 72.24 \\
                               & 1.00E-05             & 42.99    & 69.51    & 69.42          & 72.53    & 69.45 \\ \bottomrule
\end{tabular}
\end{table}
\clearpage
\subsection{APTOS}

\subsubsection{Quadratic weighted kappa}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[h]
\centering
\caption{APTOS (QWK), AlexNet}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                                                        & lr \textbackslash wd & 1.00E-03 & 1.00E-04        & 1.00E-05        & 1.00E-06        & 0      \\ \midrule
                                & 1.00E-01             & 0.0000   & 0.0000          & 0.0000          & 0.0000          & 0.0000 \\
                                & 1.00E-02             & 0.0000   & 0.0000          & 0.0000          & 0.0000          & 0.0000 \\
                                & 1.00E-03             & 0.8090   & \textbf{0.8502} & 0.8404          & 0.8333          & 0.8384 \\
\multirow{-4}{*}{SGD / Step}    & 1.00E-04             & 0.8060   & 0.7845          & 0.7868          & 0.7897          & 0.7830 \\ \midrule
                                & 1.00E-01             & 0.0000   & 0.0000          & 0.0000          & 0.0000          & 0.0000 \\
                                & 1.00E-02             & 0.0000   & 0.0000          & 0.0000          & 0.6036          & 0.0000 \\
                                & 1.00E-03             & 0.8375   & 0.8401          & \textbf{0.8494} & 0.8080          & 0.8300 \\
\multirow{-4}{*}{SGD / Cosine}  & 1.00E-04             & 0.7751   & 0.7958          & 0.7826          & 0.7928          & 0.7901 \\ \midrule
                                & 1.00E-02             & 0.0000   & 0.0128          & 0.0000          & 0.0000          & 0.0069 \\
                                & 1.00E-03             & 0.7342   & 0.7410          & 0.0000          & 0.7842          & 0.7536 \\
                                & 1.00E-04             & 0.8918   & 0.8925          & 0.8810          & \textbf{0.8945} & 0.8835 \\
\multirow{-4}{*}{Adam / Cosine} & 1.00E-05             & 0.8116   & 0.8349          & 0.8460          & 0.8541          & 0.8430 \\ \bottomrule
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{APTOS (QWK), MobileNet V3 small}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04 & 1.00E-05        & 1.00E-06        & 0               \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 0.7116   & 0.9129   & 0.9079          & 0.9205          & \textbf{0.9230} \\
                               & 1.00E-02             & 0.9175   & 0.9160   & 0.9122          & 0.9162          & 0.9136          \\
                               & 1.00E-03             & 0.8596   & 0.8701   & 0.8623          & 0.8661          & 0.8742          \\
                               & 1.00E-04             & 0.7115   & 0.6758   & 0.6748          & 0.6981          & 0.6990          \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 0.8880   & 0.9089   & 0.9050          & \textbf{0.9221} & 0.9065          \\
                               & 1.00E-02             & 0.9155   & 0.9165   & 0.9218          & 0.9076          & 0.9096          \\
                               & 1.00E-03             & 0.8405   & 0.8389   & 0.8370          & 0.8329          & 0.8353          \\
                               & 1.00E-04             & 0.6596   & 0.6840   & 0.6525          & 0.6646          & 0.6365          \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 0.7789   & 0.9075   & 0.9012          & 0.8904          & 0.8928          \\
                               & 1.00E-03             & 0.8727   & 0.9133   & \textbf{0.9183} & 0.9075          & 0.9097          \\
                               & 1.00E-04             & 0.8511   & 0.8993   & 0.9027          & 0.9002          & 0.8930          \\
                               & 1.00E-05             & 0.6245   & 0.7601   & 0.7694          & 0.7600          & 0.7441          \\ \bottomrule 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{APTOS (QWK), VGG-13 BN}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04 & 1.00E-05 & 1.00E-06        & 0               \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 0.8241   & 0.6866   & 0.8518   & 0.8336          & 0.7386          \\
                               & 1.00E-02             & 0.9147   & 0.9169   & 0.9131   & \textbf{0.9182} & 0.9115          \\
                               & 1.00E-03             & 0.8848   & 0.8922   & 0.8850   & 0.8944          & 0.8887          \\
                               & 1.00E-04             & 0.7763   & 0.7793   & 0.7779   & 0.7802          & 0.7799          \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 0.6984   & 0.8022   & 0.6942   & 0.8681          & 0.8727          \\
                               & 1.00E-02             & 0.9119   & 0.9137   & 0.9127   & 0.9172          & \textbf{0.9265} \\
                               & 1.00E-03             & 0.8834   & 0.8817   & 0.8827   & 0.8791          & 0.8857          \\
                               & 1.00E-04             & 0.7701   & 0.7762   & 0.7680   & 0.7641          & 0.7680          \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 0.5905   & 0.6594   & 0.6187   & 0.5898          & 0.4598          \\
                               & 1.00E-03             & 0.8998   & 0.9096   & 0.9235   & 0.9096          & 0.9220          \\
                               & 1.00E-04             & 0.9172   & 0.9225   & 0.9202   & 0.9145          & \textbf{0.9268} \\
                               & 1.00E-05             & 0.9005   & 0.8967   & 0.9064   & 0.9056          & 0.9116          \\ \bottomrule 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{APTOS (QWK), DeiT-tiny}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04        & 1.00E-05 & 1.00E-06        & 0               \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 0.4012   & 0.0000          & 0.0000   & 0.1017          & 0.3684          \\
                               & 1.00E-02             & 0.8818   & 0.7272          & 0.6982   & 0.7567          & 0.8190          \\
                               & 1.00E-03             & 0.8915   & \textbf{0.9037} & 0.8952   & 0.8920          & 0.8943          \\
                               & 1.00E-04             & 0.8049   & 0.7947          & 0.7878   & 0.8020          & 0.8112          \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 0.3226   & 0.3598          & 0.0674   & 0.0053          & 0.3759          \\
                               & 1.00E-02             & 0.7855   & 0.8746          & 0.8801   & 0.8059          & 0.6853          \\
                               & 1.00E-03             & 0.8957   & 0.8939          & 0.8849   & 0.8948          & \textbf{0.9032} \\
                               & 1.00E-04             & 0.7837   & 0.7976          & 0.8112   & 0.7993          & 0.8090          \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 0.6907   & 0.6163          & 0.5194   & 0.6148          & 0.4509          \\
                               & 1.00E-03             & 0.7203   & 0.6962          & 0.7201   & 0.6961          & 0.7048          \\
                               & 1.00E-04             & 0.9038   & 0.9038          & 0.8996   & \textbf{0.9130} & 0.9109          \\
                               & 1.00E-05             & 0.7882   & 0.8429          & 0.8439   & 0.8271          & 0.8635          \\ \bottomrule
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{APTOS (QWK), ResNet-50}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03        & 1.00E-04 & 1.00E-05        & 1.00E-06 & 0      \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 0.6915          & 0.6641   & 0.6376          & 0.7748   & 0.6730 \\
                               & 1.00E-02             & 0.9019          & 0.9050   & \textbf{0.9204} & 0.9128   & 0.9165 \\
                               & 1.00E-03             & 0.8958          & 0.8993   & 0.8909          & 0.8891   & 0.8983 \\
                               & 1.00E-04             & 0.7422          & 0.7663   & 0.7670          & 0.7747   & 0.7721 \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 0.6588          & 0.6160   & 0.6400          & 0.7059   & 0.6924 \\
                               & 1.00E-02             & \textbf{0.9191} & 0.9067   & 0.9137          & 0.9181   & 0.9121 \\
                               & 1.00E-03             & 0.8900          & 0.8916   & 0.8888          & 0.8924   & 0.8863 \\
                               & 1.00E-04             & 0.7585          & 0.7485   & 0.7326          & 0.7453   & 0.7388 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 0.6821          & 0.6998   & 0.7048          & 0.6930   & 0.7034 \\
                               & 1.00E-03             & 0.9106          & 0.9025   & \textbf{0.9215} & 0.9135   & 0.9129 \\
                               & 1.00E-04             & 0.9074          & 0.9140   & 0.9195          & 0.9205   & 0.9203 \\
                               & 1.00E-05             & 0.9021          & 0.9026   & 0.8978          & 0.8982   & 0.9013 \\ \bottomrule
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{APTOS (QWK), ResNet-152}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04        & 1.00E-05 & 1.00E-06        & 0               \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 0.6648   & 0.6581          & 0.6999   & 0.7025          & 0.7002          \\
                               & 1.00E-02             & 0.9159   & 0.9086          & 0.9188   & \textbf{0.9228} & 0.9194          \\
                               & 1.00E-03             & 0.9129   & 0.9093          & 0.9051   & 0.9004          & 0.9042          \\
                               & 1.00E-04             & 0.7626   & 0.7768          & 0.7695   & 0.7668          & 0.7546          \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 0.6905   & 0.7570          & 0.5382   & 0.6424          & 0.6889          \\
                               & 1.00E-02             & 0.9124   & \textbf{0.9168} & 0.9158   & 0.9163          & \textbf{0.9168} \\
                               & 1.00E-03             & 0.8810   & 0.8955          & 0.8918   & 0.8984          & 0.8932          \\
                               & 1.00E-04             & 0.7206   & 0.7364          & 0.7406   & 0.7513          & 0.7468          \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 0.7154   & 0.6978          & 0.6857   & 0.7100          & 0.7055          \\
                               & 1.00E-03             & 0.9173   & 0.9094          & 0.9150   & 0.9130          & 0.9084          \\
                               & 1.00E-04             & 0.9207   & \textbf{0.9216} & 0.9157   & 0.9175          & 0.9159          \\
                               & 1.00E-05             & 0.9086   & 0.8998          & 0.9001   & 0.9038          & 0.9114          \\ \bottomrule
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{APTOS (QWK), DeiT-small}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03        & 1.00E-04        & 1.00E-05        & 1.00E-06 & 0      \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 0.0000          & 0.0000          & 0.0835          & 0.3879   & 0.0000 \\
                               & 1.00E-02             & 0.8714          & 0.8797          & 0.8926          & 0.8790   & 0.8949 \\
                               & 1.00E-03             & \textbf{0.9032} & 0.9017          & 0.8998          & 0.8938   & 0.8995 \\
                               & 1.00E-04             & 0.7765          & 0.7724          & 0.7753          & 0.7812   & 0.7781 \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 0.0000          & 0.0000          & 0.0000          & 0.0000   & 0.0000 \\
                               & 1.00E-02             & 0.7242          & 0.8027          & \textbf{0.9057} & 0.7573   & 0.7013 \\
                               & 1.00E-03             & 0.8950          & 0.8888          & 0.8974          & 0.8969   & 0.9040 \\
                               & 1.00E-04             & 0.7883          & 0.7648          & 0.7671          & 0.7745   & 0.7796 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 0.6299          & 0.4583          & 0.3939          & 0.3875   & 0.3517 \\
                               & 1.00E-03             & 0.7182          & 0.7176          & 0.7183          & 0.6900   & 0.7019 \\
                               & 1.00E-04             & 0.9058          & \textbf{0.9205} & 0.9197          & 0.9162   & 0.9179 \\
                               & 1.00E-05             & 0.7975          & 0.8890          & 0.8754          & 0.8569   & 0.8815 \\ \bottomrule 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{APTOS (QWK), PNASNet-5 large}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03        & 1.00E-04        & 1.00E-05 & 1.00E-06 & 0               \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 0.9244          & 0.9193          & 0.9127   & 0.9233   & \textbf{0.9271} \\
                               & 1.00E-02             & 0.9043          & 0.9073          & 0.9068   & 0.9028   & 0.8930          \\
                               & 1.00E-03             & 0.8757          & 0.8749          & 0.8686   & 0.8689   & 0.8695          \\
                               & 1.00E-04             & 0.7007          & 0.7255          & 0.7219   & 0.7191   & 0.6924          \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & \textbf{0.9153} & 0.9121          & 0.9139   & 0.9121   & 0.9082          \\
                               & 1.00E-02             & 0.9026          & 0.9059          & 0.9088   & 0.8939   & 0.8972          \\
                               & 1.00E-03             & 0.8547          & 0.8514          & 0.8479   & 0.8659   & 0.8597          \\
                               & 1.00E-04             & 0.6906          & 0.6525          & 0.6776   & 0.6604   & 0.6931          \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 0.6615          & 0.5603          & 0.6999   & 0.7993   & 0.6967          \\
                               & 1.00E-03             & 0.9227          & \textbf{0.9236} & 0.9126   & 0.9203   & 0.9203          \\
                               & 1.00E-04             & 0.9122          & 0.9127          & 0.9064   & 0.9101   & 0.9145          \\
                               & 1.00E-05             & 0.8946          & 0.8938          & 0.8893   & 0.8928   & 0.8955          \\ \bottomrule
\end{tabular}
\end{table}
\clearpage
\subsubsection{Accuracy}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{APTOS (Accuracy), AlexNet}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04 & 1.00E-05       & 1.00E-06 & 0              \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 49.38    & 49.38    & 49.38          & 49.38    & 49.38          \\
                               & 1.00E-02             & 49.38    & 49.38    & 49.38          & 49.38    & 49.38          \\
                               & 1.00E-03             & 76.88    & 79.48    & 78.93          & 79.34    & \textbf{79.62} \\
                               & 1.00E-04             & 76.06    & 76.88    & 76.74          & 76.47    & 76.74          \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 49.38    & 49.38    & 49.38          & 49.38    & 49.38          \\
                               & 1.00E-02             & 49.38    & 49.38    & 49.38          & 70.59    & 49.38          \\
                               & 1.00E-03             & 79.21    & 78.11    & \textbf{79.34} & 77.02    & 78.66          \\
                               & 1.00E-04             & 77.29    & 76.61    & 77.29          & 76.74    & 76.33          \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 49.38    & 49.38    & 49.38          & 49.38    & 49.38          \\
                               & 1.00E-03             & 74.01    & 73.32    & 49.38          & 76.20    & 73.87          \\
                               & 1.00E-04             & 83.45    & 82.90    & 83.45          & 82.49    & \textbf{83.58} \\
                               & 1.00E-05             & 77.29    & 78.39    & 78.93          & 79.89    & 79.48          \\ \bottomrule 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{APTOS (Accuracy), MobileNet V3 small}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04       & 1.00E-05 & 1.00E-06       & 0              \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 62.65    & 85.50          & 84.27    & 85.64          & \textbf{86.32} \\
                               & 1.00E-02             & 85.64    & 85.50          & 84.82    & 84.95          & 86.18          \\
                               & 1.00E-03             & 80.85    & 80.03          & 80.57    & 80.30          & 81.12          \\
                               & 1.00E-04             & 71.96    & 71.14          & 70.18    & 71.55          & 71.14          \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 83.04    & 85.23          & 84.82    & \textbf{86.59} & 84.40          \\
                               & 1.00E-02             & 84.82    & 85.64          & 85.77    & 85.09          & 84.54          \\
                               & 1.00E-03             & 78.93    & 79.21          & 79.75    & 78.39          & 79.75          \\
                               & 1.00E-04             & 68.26    & 70.59          & 69.90    & 69.77          & 69.08          \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 65.53    & 83.99          & 83.04    & 83.31          & 82.76          \\
                               & 1.00E-03             & 78.66    & \textbf{85.09} & 83.86    & 84.27          & 84.40          \\
                               & 1.00E-04             & 78.25    & 83.86          & 83.45    & 82.90          & 83.45          \\
                               & 1.00E-05             & 61.29    & 73.87          & 74.69    & 74.15          & 73.87          \\ \bottomrule
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{APTOS (Accuracy), VGG-13 BN}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04 & 1.00E-05       & 1.00E-06 & 0              \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 78.52    & 72.50    & 79.07          & 78.39    & 74.28          \\
                               & 1.00E-02             & 85.36    & 85.50    & \textbf{86.32} & 85.77    & 85.50          \\
                               & 1.00E-03             & 82.76    & 84.27    & 83.17          & 84.13    & 83.99          \\
                               & 1.00E-04             & 75.51    & 75.10    & 75.24          & 75.24    & 75.51          \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 72.50    & 78.11    & 71.68          & 81.26    & 80.03          \\
                               & 1.00E-02             & 85.09    & 85.23    & 84.82          & 85.77    & \textbf{86.18} \\
                               & 1.00E-03             & 83.17    & 83.17    & 82.49          & 82.63    & 82.90          \\
                               & 1.00E-04             & 74.56    & 74.56    & 74.42          & 74.56    & 74.42          \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 65.80    & 67.31    & 69.77          & 66.21    & 60.74          \\
                               & 1.00E-03             & 84.27    & 84.68    & 85.91          & 84.27    & 85.77          \\
                               & 1.00E-04             & 85.50    & 85.77    & 85.09          & 86.05    & \textbf{86.18} \\
                               & 1.00E-05             & 83.99    & 83.72    & 83.58          & 83.17    & 84.54          \\ \bottomrule
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{APTOS (Accuracy), DeiT-tiny}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04 & 1.00E-05 & 1.00E-06       & 0              \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 58.97    & 49.18    & 10.60    & 49.18          & 59.24          \\
                               & 1.00E-02             & 82.88    & 74.05    & 72.28    & 74.59          & 75.82          \\
                               & 1.00E-03             & 83.29    & 83.56    & 83.42    & 83.42          & \textbf{84.38} \\
                               & 1.00E-04             & 76.22    & 76.22    & 76.22    & 77.85          & 77.31          \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 56.66    & 56.52    & 49.46    & 49.18          & 57.61          \\
                               & 1.00E-02             & 74.73    & 80.43    & 82.07    & 77.17          & 72.69          \\
                               & 1.00E-03             & 83.56    & 83.70    & 81.93    & 82.20          & \textbf{84.51} \\
                               & 1.00E-04             & 76.22    & 76.36    & 76.90    & 77.72          & 76.49          \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 71.47    & 68.89    & 63.72    & 68.07          & 60.33          \\
                               & 1.00E-03             & 72.69    & 71.88    & 71.60    & 72.01          & 73.51          \\
                               & 1.00E-04             & 83.72    & 85.09    & 84.68    & \textbf{85.64} & \textbf{85.64} \\
                               & 1.00E-05             & 76.09    & 78.53    & 80.30    & 78.94          & 80.43          \\ \bottomrule 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{APTOS (Accuracy), ResNet-50}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04       & 1.00E-05       & 1.00E-06 & 0              \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 71.55    & 71.27          & 70.86          & 75.38    & 71.27          \\
                               & 1.00E-02             & 84.82    & 84.82          & 85.23          & 84.82    & \textbf{85.77} \\
                               & 1.00E-03             & 83.72    & 83.86          & 83.58          & 84.27    & 83.86          \\
                               & 1.00E-04             & 74.15    & 74.01          & 74.56          & 74.97    & 74.28          \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 69.90    & 68.67          & 70.45          & 72.23    & 72.09          \\
                               & 1.00E-02             & 84.54    & \textbf{85.23} & 84.95          & 84.68    & 84.68          \\
                               & 1.00E-03             & 83.17    & 83.99          & 83.45          & 82.90    & 82.49          \\
                               & 1.00E-04             & 73.73    & 73.87          & 73.60          & 73.73    & 73.60          \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 72.37    & 72.09          & 73.46          & 73.46    & 73.60          \\
                               & 1.00E-03             & 85.64    & 84.27          & \textbf{86.87} & 85.36    & 85.09          \\
                               & 1.00E-04             & 85.09    & 85.36          & 85.64          & 86.05    & 85.77          \\
                               & 1.00E-05             & 85.50    & 84.95          & 83.86          & 84.40    & 85.50          \\ \bottomrule 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{APTOS (Accuracy), ResNet-152}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04 & 1.00E-05       & 1.00E-06       & 0              \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 71.82    & 71.55    & 72.09          & 72.64          & 72.50          \\
                               & 1.00E-02             & 85.23    & 84.40    & 84.95          & \textbf{85.77} & 85.23          \\
                               & 1.00E-03             & 84.68    & 84.95    & 84.68          & 83.72          & 84.82          \\
                               & 1.00E-04             & 74.83    & 75.38    & 75.24          & 75.24          & 74.69          \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 72.37    & 75.65    & 66.48          & 70.45          & 73.05          \\
                               & 1.00E-02             & 84.82    & 84.82    & 84.82          & 85.09          & \textbf{85.77} \\
                               & 1.00E-03             & 83.58    & 83.72    & 83.45          & 84.40          & 83.58          \\
                               & 1.00E-04             & 73.73    & 74.01    & 73.87          & 74.42          & 74.56          \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 71.27    & 71.96    & 72.37          & 72.64          & 72.50          \\
                               & 1.00E-03             & 85.50    & 85.50    & \textbf{86.18} & \textbf{86.18} & 85.09          \\
                               & 1.00E-04             & 85.36    & 85.23    & 85.36          & \textbf{86.18} & 84.95          \\
                               & 1.00E-05             & 83.72    & 84.54    & 83.99          & 83.58          & 83.58          \\ \bottomrule 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{APTOS (Accuracy), DeiT-small}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04       & 1.00E-05       & 1.00E-06       & 0     \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 0.00     & 27.31          & 49.18          & 57.47          & 10.19 \\
                               & 1.00E-02             & 81.25    & 81.52          & 83.02          & 83.15          & 82.61 \\
                               & 1.00E-03             & 82.74    & 83.97          & \textbf{84.38} & 82.74          & 83.15 \\
                               & 1.00E-04             & 75.00    & 74.46          & 74.86          & 75.00          & 75.54 \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 49.18    & 49.18          & 5.30           & 49.18          & 49.18 \\
                               & 1.00E-02             & 72.83    & 75.95          & 83.56          & 74.05          & 72.96 \\
                               & 1.00E-03             & 82.07    & 82.74          & 84.10          & \textbf{85.33} & 84.10 \\
                               & 1.00E-04             & 75.00    & 73.91          & 74.05          & 74.05          & 75.00 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 70.11    & 60.73          & 57.47          & 58.83          & 56.39 \\
                               & 1.00E-03             & 72.83    & 72.42          & 72.15          & 72.15          & 71.06 \\
                               & 1.00E-04             & 84.68    & \textbf{86.05} & 85.64          & 85.09          & 85.36 \\
                               & 1.00E-05             & 76.63    & 83.29          & 82.07          & 80.98          & 82.61 \\ \bottomrule 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{APTOS (Accuracy), PNASNet-5 large}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03       & 1.00E-04       & 1.00E-05 & 1.00E-06 & 0     \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & \textbf{86.59} & 85.64          & 85.64    & 85.64    & 85.91 \\
                               & 1.00E-02             & 83.45          & 84.27          & 84.54    & 83.31    & 83.72 \\
                               & 1.00E-03             & 81.94          & 81.26          & 82.22    & 80.98    & 81.53 \\
                               & 1.00E-04             & 72.37          & 72.78          & 72.50    & 72.50    & 72.91 \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & \textbf{85.50} & 84.95          & 85.36    & 84.68    & 85.09 \\
                               & 1.00E-02             & 83.17          & 85.23          & 83.86    & 83.31    & 82.63 \\
                               & 1.00E-03             & 80.44          & 81.53          & 80.30    & 80.98    & 80.85 \\
                               & 1.00E-04             & 71.27          & 70.59          & 71.14    & 70.31    & 71.68 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 67.44          & 68.81          & 72.37    & 75.10    & 71.00 \\
                               & 1.00E-03             & 85.09          & \textbf{86.73} & 85.77    & 85.91    & 85.77 \\
                               & 1.00E-04             & 85.91          & 84.95          & 84.95    & 85.77    & 84.95 \\
                               & 1.00E-05             & 82.76          & 82.76          & 83.04    & 82.63    & 82.76 \\ \bottomrule 
\end{tabular}
\end{table}

\clearpage

\subsection{Human Protein Atlas}
Entries are macro F1 score on the validation set (5,664 images), and then using the thresholds found with the validation set, macro F1 score on the test validation set (2,826 images).

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{Human Protein Atlas, AlexNet}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                                                                         & lr \textbackslash wd & 1.00E-03        & 1.00E-04                 & 1.00E-05                 & 1.00E-06                 & 0               \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SGD /\\ Step\end{tabular}}    & 1.00E-01             & 0.1069 / 0.1078 & \textbf{0.2957 / 0.2805} & 0.2956 / 0.3058          & 0.2918 / 0.2955          & 0.2916 / 0.2882 \\
                                                                         & 1.00E-02             & 0.1988 / 0.1938 & 0.2064 / 0.1967          & 0.1927 / 0.1924          & 0.1978 / 0.1864          & 0.1892 / 0.1830 \\
                                                                         & 1.00E-03             & 0.0970 / 0.0980 & 0.0877 / 0.0905          & 0.1041 / 0.0971          & 0.0902 / 0.0903          & 0.1002 / 0.0984 \\
                                                                         & 1.00E-04             & 0.0466 / 0.0458 & 0.0461 / 0.0480          & 0.0474 / 0.0484          & 0.0418 / 0.0429          & 0.0449 / 0.0453 \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SGD /\\ Cosine\end{tabular}}  & 1.00E-01             & 0.1049 / 0.1060 & 0.2841 / 0.2811          & 0.2873 / 0.2870          & \textbf{0.2928 / 0.2960} & 0.2798 / 0.2756 \\
                                                                         & 1.00E-02             & 0.1951 / 0.1903 & 0.1963 / 0.1908          & 0.1941 / 0.1901          & 0.1939 / 0.1943          & 0.2029 / 0.1981 \\
                                                                         & 1.00E-03             & 0.0914 / 0.0852 & 0.0960 / 0.0922          & 0.0947 / 0.0983          & 0.0955 / 0.0990          & 0.0987 / 0.0950 \\
                                                                         & 1.00E-04             & 0.0477 / 0.0465 & 0.0455 / 0.0474          & 0.0439 / 0.0453          & 0.0489 / 0.0528          & 0.0482 / 0.0486 \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Adam /\\ Cosine\end{tabular}} & 1.00E-02             & 0.0209 / 0.0209 & 0.0209 / 0.0209          & 0.0209 / 0.0209          & 0.0209 / 0.0209          & 0.0209 / 0.0209 \\
                                                                         & 1.00E-03             & 0.2912 / 0.2916 & 0.2926 / 0.2869          & 0.0209 / 0.0209          & 0.0209 / 0.0209          & 0.2966 / 0.2995 \\
                                                                         & 1.00E-04             & 0.2582 / 0.2638 & 0.3842 / 0.3400          & \textbf{0.3846 / 0.3699} & 0.3743 / 0.3799          & 0.3472 / 0.3531 \\
                                                                         & 1.00E-05             & 0.0448 / 0.0471 & 0.2265 / 0.2167          & 0.2173 / 0.2119          & 0.2243 / 0.2276          & 0.2220 / 0.2166 \\ \bottomrule
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{Human Protein Atlas, MobileNet V3 small}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                                                                         & lr \textbackslash wd & 1.00E-03        & 1.00E-04        & 1.00E-05                 & 1.00E-06                 & 0               \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SGD /\\ Step\end{tabular}}    & 1.00E-01             & 0.0460 / 0.0489 & 0.3649 / 0.3644 & 0.3952 / 0.3689          & \textbf{0.4012 / 0.3849} & 0.3825 / 0.3804 \\
                                                                         & 1.00E-02             & 0.1561 / 0.1540 & 0.1735 / 0.1694 & 0.1805 / 0.1767          & 0.1772 / 0.1759          & 0.1811 / 0.1819 \\
                                                                         & 1.00E-03             & 0.0698 / 0.0724 & 0.0612 / 0.0615 & 0.0618 / 0.0602          & 0.0630 / 0.0639          & 0.0585 / 0.0610 \\
                                                                         & 1.00E-04             & 0.0411 / 0.0459 & 0.0455 / 0.0483 & 0.0431 / 0.0444          & 0.0490 / 0.0405          & 0.0431 / 0.0379 \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SGD /\\ Cosine\end{tabular}}  & 1.00E-01             & 0.0550 / 0.0547 & 0.3798 / 0.3822 & \textbf{0.4169 / 0.3816} & 0.3974 / 0.3795          & 0.3876 / 0.3705 \\
                                                                         & 1.00E-02             & 0.1570 / 0.1499 & 0.1803 / 0.1768 & 0.1713 / 0.1676          & 0.1811 / 0.1811          & 0.1819 / 0.1781 \\
                                                                         & 1.00E-03             & 0.0567 / 0.0580 & 0.0606 / 0.0633 & 0.0610 / 0.0613          & 0.0618 / 0.0657          & 0.0612 / 0.0611 \\
                                                                         & 1.00E-04             & 0.0450 / 0.0466 & 0.0381 / 0.0431 & 0.0444 / 0.0422          & 0.0474 / 0.0474          & 0.0481 / 0.0492 \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Adam /\\ Cosine\end{tabular}} & 1.00E-02             & 0.5261 / 0.5124 & 0.6086 / 0.5771 & 0.6011 / 0.5544          & 0.5785 / 0.5724          & 0.6096 / 0.5658 \\
                                                                         & 1.00E-03             & 0.4112 / 0.3919 & 0.6066 / 0.604  & 0.6051 / 0.5744          & \textbf{0.6108 / 0.5608} & 0.5999 / 0.5929 \\
                                                                         & 1.00E-04             & 0.0560 / 0.0588 & 0.4531 / 0.4085 & 0.4512 / 0.4416          & 0.4492 / 0.4314          & 0.4550 / 0.4412 \\
                                                                         & 1.00E-05             & 0.0209 / 0.0209 & 0.1622 / 0.1560 & 0.1747 / 0.1800          & 0.1799 / 0.1799          & 0.1692 / 0.1787 \\ \bottomrule 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
\centering
\caption{Human Protein Atlas, VGG-13 BN}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                                                        & lr \textbackslash wd & 1.00E-03        & 1.00E-04                 & 1.00E-05                 & 1.00E-06        & 0               \\ \midrule
\begin{tabular}[c]{@{}l@{}}SGD /\\ Step\end{tabular}    & 1.00E-01             & 0.4395 / 0.4282 & 0.5941 / 0.5228          & \textbf{0.5961 / 0.5271} & 0.5901 / 0.5564 & 0.5919 / 0.5630 \\
                                                        & 1.00E-02             & 0.3251 / 0.3163 & 0.3305 / 0.3190          & 0.3251 / 0.3212          & 0.3264 / 0.3175 & 0.3247 / 0.3179 \\
                                                        & 1.00E-03             & 0.1281 / 0.1245 & 0.1286 / 0.1296          & 0.1283 / 0.1262          & 0.1249 / 0.1177 & 0.1245 / 0.1265 \\
                                                        & 1.00E-04             & 0.0390 / 0.0371 & 0.0392 / 0.0395          & 0.0398 / 0.0426          & 0.0380 / 0.0385 & 0.0362 / 0.0377 \\ \midrule
\begin{tabular}[c]{@{}l@{}}SGD /\\ Cosine\end{tabular}  & 1.00E-01             & 0.4539 / 0.4418 & \textbf{0.6016 / 0.5489} & 0.6012 / 0.5439          & 0.5910 / 0.5394 & 0.6009 / 0.5454 \\
                                                        & 1.00E-02             & 0.3198 / 0.3178 & 0.3317 / 0.3290          & 0.3298 / 0.3169          & 0.3211 / 0.3092 & 0.3204 / 0.3181 \\
                                                        & 1.00E-03             & 0.1270 / 0.1232 & 0.1336 / 0.1229          & 0.1298 / 0.1258          & 0.1304 / 0.1241 & 0.1241 / 0.1216 \\
                                                        & 1.00E-04             & 0.0336 / 0.0375 & 0.0372 / 0.0366          & 0.0357 / 0.0354          & 0.0368 / 0.0356 & 0.0378 / 0.0398 \\ \midrule
\begin{tabular}[c]{@{}l@{}}Adam /\\ Cosine\end{tabular} & 1.00E-02             & 0.2723 / 0.2578 & 0.0391 / 0.0401          & 0.1128 / 0.1091          & 0.0384 / 0.0391 & 0.0689 / 0.0691 \\
                                                        & 1.00E-03             & 0.6368 / 0.5927 & 0.6396 / 0.6058          & 0.5851 / 0.5734          & 0.6010 / 0.5566 & 0.6018 / 0.5618 \\
                                                        & 1.00E-04             & 0.6356 / 0.6414 & 0.6749 / 0.6590          & \textbf{0.6794 / 0.6493} & 0.6681 / 0.6298 & 0.6559 / 0.6399 \\
                                                        & 1.00E-05             & 0.2732 / 0.2646 & 0.3785 / 0.3724          & 0.3722 / 0.3683          & 0.3665 / 0.3903 & 0.3703 / 0.3932 \\ \bottomrule
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{Human Protein Atlas, DeiT-tiny}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                                                                         & lr \textbackslash wd & 1.00E-03        & 1.00E-04                 & 1.00E-05        & 1.00E-06                 & 0               \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SGD /\\ Step\end{tabular}}    & 1.00E-01             & 0.0532 / 0.0539 & 0.5017 / 0.4673          & 0.4857 / 0.4876 & \textbf{0.5019 / 0.4730} & 0.4992 / 0.4915 \\
                                                                         & 1.00E-02             & 0.2739 / 0.2604 & 0.3169 / 0.3083          & 0.3336 / 0.3195 & 0.3244 / 0.3191          & 0.3448 / 0.3380 \\
                                                                         & 1.00E-03             & 0.1263 / 0.1240 & 0.1397 / 0.1385          & 0.1138 / 0.1132 & 0.1290 / 0.1188          & 0.1284 / 0.1339 \\
                                                                         & 1.00E-04             & 0.0387 / 0.0390 & 0.0396 / 0.0414          & 0.0336 / 0.0355 & 0.0343 / 0.0359          & 0.0332 / 0.0345 \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SGD /\\ Cosine\end{tabular}}  & 1.00E-01             & 0.0576 / 0.0559 & 0.5068 / 0.4632          & 0.4962 / 0.4808 & \textbf{0.5387 / 0.5119} & 0.4977 / 0.4844 \\
                                                                         & 1.00E-02             & 0.2723 / 0.2637 & 0.3446 / 0.3255          & 0.3291 / 0.3231 & 0.3345 / 0.3305          & 0.3246 / 0.3128 \\
                                                                         & 1.00E-03             & 0.1206 / 0.1255 & 0.1269 / 0.1371          & 0.1247 / 0.1295 & 0.1304 / 0.1331          & 0.1064 / 0.1062 \\
                                                                         & 1.00E-04             & 0.0371 / 0.0385 & 0.0317 / 0.0342          & 0.0380 / 0.0406 & 0.0393 / 0.0411          & 0.0343 / 0.0351 \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Adam /\\ Cosine\end{tabular}} & 1.00E-02             & 0.2721 / 0.2724 & 0.0832 / 0.0765          & 0.0629 / 0.0620 & 0.0822 / 0.0804          & 0.0722 / 0.0711 \\
                                                                         & 1.00E-03             & 0.2668 / 0.2555 & 0.5237 / 0.5056          & 0.4927 / 0.5205 & 0.5170 / 0.4651          & 0.5147 / 0.4828 \\
                                                                         & 1.00E-04             & 0.0555 / 0.0567 & \textbf{0.5777 / 0.5358} & 0.5628 / 0.4997 & 0.5571 / 0.5285          & 0.5407 / 0.5073 \\
                                                                         & 1.00E-05             & 0.0209 / 0.0209 & 0.2881 / 0.2686          & 0.3545 / 0.3604 & 0.3408 / 0.3290          & 0.3368 / 0.3336 \\ \bottomrule 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{Human Protein Atlas, ResNet-50}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                                                                         & lr \textbackslash wd & 1.00E-03        & 1.00E-04        & 1.00E-05                 & 1.00E-06                 & 0                        \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SGD /\\ Step\end{tabular}}    & 1.00E-01             & 0.4107 / 0.4096 & 0.5778 / 0.6015 & 0.6034 / 0.5650          & \textbf{0.6146 / 0.5566} & 0.6129 / 0.5939          \\
                                                                         & 1.00E-02             & 0.3096 / 0.3184 & 0.3049 / 0.3034 & 0.3032 / 0.3066          & 0.3041 / 0.3006          & 0.3024 / 0.3057          \\
                                                                         & 1.00E-03             & 0.0826 / 0.0884 & 0.0950 / 0.0943 & 0.0892 / 0.0889          & 0.0945 / 0.0961          & 0.0920 / 0.0946          \\
                                                                         & 1.00E-04             & 0.0311 / 0.0319 & 0.0324 / 0.0329 & 0.0321 / 0.0321          & 0.0309 / 0.0314          & 0.0332 / 0.0344          \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SGD /\\ Cosine\end{tabular}}  & 1.00E-01             & 0.4356 / 0.4303 & 0.6189 / 0.5747 & 0.6207 / 0.6040          & 0.5963 / 0.5690          & \textbf{0.6233 / 0.5931} \\
                                                                         & 1.00E-02             & 0.3119 / 0.3067 & 0.3061 / 0.3023 & 0.3020 / 0.3075          & 0.2957 / 0.3045          & 0.3033 / 0.3019          \\
                                                                         & 1.00E-03             & 0.0877 / 0.0890 & 0.0887 / 0.0852 & 0.0879 / 0.0923          & 0.0838 / 0.0842          & 0.0878 / 0.0852          \\
                                                                         & 1.00E-04             & 0.0311 / 0.0322 & 0.0318 / 0.0320 & 0.0294 / 0.0292          & 0.0341 / 0.0351          & 0.0310 / 0.0312          \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Adam /\\ Cosine\end{tabular}} & 1.00E-02             & 0.4899 / 0.4877 & 0.4725 / 0.4479 & 0.4819 / 0.4576          & 0.4356 / 0.4243          & 0.4263 / 0.4461          \\
                                                                         & 1.00E-03             & 0.6092 / 0.6088 & 0.6683 / 0.6439 & \textbf{0.6718 / 0.6502} & 0.6656 / 0.6397          & 0.6540 / 0.6544          \\
                                                                         & 1.00E-04             & 0.5209 / 0.5203 & 0.6585 / 0.6109 & 0.6627 / 0.6404          & 0.6615 / 0.6468          & 0.6370 / 0.6507          \\
                                                                         & 1.00E-05             & 0.0256 / 0.0253 & 0.4405 / 0.4282 & 0.4298 / 0.4240          & 0.4379 / 0.4266          & 0.4528 / 0.4282          \\ \bottomrule
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{Human Protein Atlas, ResNet-152}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                                                                         & lr \textbackslash wd & 1.00E-03        & 1.00E-04        & 1.00E-05                 & 1.00E-06        & 0                        \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SGD /\\ Step\end{tabular}}    & 1.00E-01             & 0.4077 / 0.3993 & 0.5765 / 0.5696 & \textbf{0.5879 / 0.5584} & 0.5856 / 0.5421 & 0.5733 / 0.5396          \\
                                                                         & 1.00E-02             & 0.3158 / 0.3143 & 0.3121 / 0.3063 & 0.3117 / 0.3112          & 0.3123 / 0.3124 & 0.2957 / 0.2963          \\
                                                                         & 1.00E-03             & 0.0965 / 0.0996 & 0.1011 / 0.1011 & 0.0969 / 0.0959          & 0.1035 / 0.1027 & 0.1010 / 0.0969          \\
                                                                         & 1.00E-04             & 0.0335 / 0.0342 & 0.0332 / 0.0345 & 0.0296 / 0.0297          & 0.0322 / 0.0331 & 0.0351 / 0.0346          \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SGD /\\ Cosine\end{tabular}}  & 1.00E-01             & 0.4248 / 0.4284 & 0.5719 / 0.5876 & 0.5710 / 0.5480          & 0.5860 / 0.5508 & \textbf{0.6018 / 0.5570} \\
                                                                         & 1.00E-02             & 0.3144 / 0.3132 & 0.3126 / 0.3076 & 0.3050 / 0.3063          & 0.3064 / 0.3042 & 0.3078 / 0.3097          \\
                                                                         & 1.00E-03             & 0.0914 / 0.0996 & 0.0974 / 0.1010 & 0.1026 / 0.0982          & 0.0962 / 0.0919 & 0.1028 / 0.1007          \\
                                                                         & 1.00E-04             & 0.0347 / 0.0352 & 0.0277 / 0.0291 & 0.0343 / 0.0351          & 0.0325 / 0.0342 & 0.0354 / 0.0358          \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Adam /\\ Cosine\end{tabular}} & 1.00E-02             & 0.4609 / 0.4665 & 0.3658 / 0.3695 & 0.4213 / 0.4251          & 0.3374 / 0.3329 & 0.4380 /  0.4720         \\
                                                                         & 1.00E-03             & 0.6115 / 0.6233 & 0.6571 / 0.6157 & 0.6544 / 0.6422          & 0.6363 / 0.6228 & \textbf{0.6732 / 0.6505} \\
                                                                         & 1.00E-04             & 0.5356 / 0.5254 & 0.6182 / 0.6039 & 0.6349 / 0.6013          & 0.6456 / 0.6236 & 0.6202 / 0.6316          \\
                                                                         & 1.00E-05             & 0.0292 / 0.0285 & 0.4648 / 0.4427 & 0.4711 / 0.4573          & 0.4685 / 0.4450 & 0.4598 / 0.4357          \\ \bottomrule 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{Human Protein Atlas, DeiT-small}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                                                                         & lr \textbackslash wd & 1.00E-03        & 1.00E-04                 & 1.00E-05        & 1.00E-06                 & 0                        \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SGD /\\ Step\end{tabular}}    & 1.00E-01             & 0.0488 / 0.0502 & 0.4905 / 0.5035          & 0.4874 / 0.4676 & \textbf{0.5230 / 0.5147} & 0.5185 / 0.5050          \\
                                                                         & 1.00E-02             & 0.2780 / 0.2703 & 0.3349 / 0.3321          & 0.3435 / 0.3159 & 0.3338 / 0.3275          & 0.3304 / 0.3301          \\
                                                                         & 1.00E-03             & 0.1331 / 0.1320 & 0.1212 / 0.1223          & 0.1240 / 0.1170 & 0.1330 / 0.1373          & 0.1354 / 0.1388          \\
                                                                         & 1.00E-04             & 0.0371 / 0.0392 & 0.0366 / 0.0360          & 0.0351 / 0.0345 & 0.0363 / 0.0364          & 0.0387 / 0.0391          \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SGD /\\ Cosine\end{tabular}}  & 1.00E-01             & 0.0502 / 0.0500 & 0.4988 / 0.4759          & 0.5163 / 0.4530 & 0.5081 / 0.4624          & \textbf{0.5329 / 0.5072} \\
                                                                         & 1.00E-02             & 0.2849 / 0.2643 & 0.3425 / 0.3311          & 0.3424 / 0.3403 & 0.3417 / 0.3473          & 0.3342 / 0.3294          \\
                                                                         & 1.00E-03             & 0.1185 / 0.1189 & 0.1204 / 0.1267          & 0.1340 / 0.1350 & 0.1275 / 0.1269          & 0.1383 / 0.1340          \\
                                                                         & 1.00E-04             & 0.0353 / 0.0365 & 0.0368 / 0.0371          & 0.0372 / 0.0394 & 0.0373 / 0.0383          & 0.0349 / 0.0342          \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Adam /\\ Cosine\end{tabular}} & 1.00E-02             & 0.2451 / 0.2363 & 0.0844 / 0.0831          & 0.0744 / 0.0748 & 0.0819 / 0.0826          & 0.0587 / 0.0627          \\
                                                                         & 1.00E-03             & 0.2839 / 0.2748 & 0.5357 / 0.5253          & 0.5048 / 0.4706 & 0.5425 / 0.5333          & 0.5446 / 0.5231          \\
                                                                         & 1.00E-04             & 0.0697 / 0.0725 & \textbf{0.6148 / 0.5959} & 0.5812 / 0.5881 & 0.5819 / 0.5627          & 0.6009 / 0.5650          \\
                                                                         & 1.00E-05             & 0.0209 / 0.0209 & 0.3388 / 0.3388          & 0.4029 / 0.3996 & 0.4090 / 0.4386          & 0.4275 / 0.4131          \\ \bottomrule
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{Human Protein Atlas, PNASNet-5 large}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                                                                         & lr \textbackslash wd & 1.00E-03        & 1.00E-04                 & 1.00E-05                 & 1.00E-06        & 0               \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SGD /\\ Step\end{tabular}}    & 1.00E-01             & 0.3496 / 0.3317 & \textbf{0.5325 / 0.5073} & 0.5153 / 0.5009          & 0.5057 / 0.4673 & 0.5220 / 0.4721 \\
                                                                         & 1.00E-02             & 0.2551 / 0.2522 & 0.2271 / 0.2154          & 0.2244 / 0.2123          & 0.2253 / 0.2197 & 0.2344 / 0.2282 \\
                                                                         & 1.00E-03             & 0.0761 / 0.0733 & 0.0834 / 0.0784          & 0.0785 / 0.0836          & 0.0763 / 0.0800 & 0.0776 / 0.0785 \\
                                                                         & 1.00E-04             & 0.0316 / 0.0294 & 0.0301 / 0.0316          & 0.0299 / 0.0289          & 0.0309 / 0.0313 & 0.0293 / 0.0297 \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}SGD /\\ Cosine\end{tabular}}  & 1.00E-01             & 0.3651 / 0.3532 & \textbf{0.5437 / 0.5211} & 0.5154 / 0.4866          & 0.5054 / 0.4900 & 0.4977 / 0.4687 \\
                                                                         & 1.00E-02             & 0.2573 / 0.2471 & 0.2252 / 0.2233          & 0.2266 / 0.2149          & 0.2214 / 0.2152 & 0.2265 / 0.2122 \\
                                                                         & 1.00E-03             & 0.0747 / 0.0770 & 0.0713 / 0.0764          & 0.0715 / 0.0747          & 0.0735 / 0.0728 & 0.0708 / 0.0722 \\
                                                                         & 1.00E-04             & 0.0312 / 0.0322 & 0.0334 / 0.0334          & 0.0314 / 0.0316          & 0.0312 / 0.0342 & 0.0307 / 0.0334 \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Adam /\\ Cosine\end{tabular}} & 1.00E-02             & 0.5437 / 0.5627 & 0.5376 / 0.5302          & 0.5188 / 0.4895          & 0.4593 / 0.4503 & 0.4277 / 0.4279 \\
                                                                         & 1.00E-03             & 0.6881 / 0.6785 & 0.6816 / 0.6521          & \textbf{0.6941 / 0.6873} & 0.6886 / 0.6717 & 0.6763 / 0.6599 \\
                                                                         & 1.00E-04             & 0.4398 / 0.4397 & 0.6409 / 0.6448          & 0.6435 / 0.6144          & 0.6165 / 0.6162 & 0.6335 / 0.6242 \\
                                                                         & 1.00E-05             & 0.0209 / 0.0209 & 0.4505 / 0.4407          & 0.4317 / 0.4143          & 0.4375 / 0.4100 & 0.4374 / 0.4331 \\ \bottomrule 
\end{tabular}
\end{table}


\clearpage


\subsection{SIIM-ISIC Melanoma}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{SIIM-ISIC Melanoma, AlexNet}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04        & 1.00E-05        & 1.00E-06 & 0               \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 0.0000   & 0.0000          & 0.0000          & 0.0000   & 0.0000          \\
                               & 1.00E-02             & 0.9023   & 0.9044          & \textbf{0.9074} & 0.9065   & 0.9068          \\
                               & 1.00E-03             & 0.8994   & 0.8978          & 0.8984          & 0.9008   & 0.9018          \\
                               & 1.00E-04             & 0.8691   & 0.8685          & 0.8627          & 0.8731   & 0.8647          \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 0.0000   & 0.0000          & 0.0000          & 0.0000   & 0.0000          \\
                               & 1.00E-02             & 0.8931   & 0.9050          & 0.9124          & 0.9076   & \textbf{0.9126} \\
                               & 1.00E-03             & 0.8989   & 0.8983          & 0.8992          & 0.8996   & 0.8994          \\
                               & 1.00E-04             & 0.8669   & 0.8697          & 0.8698          & 0.8673   & 0.8652          \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 0.5116   & 0.5043          & 0.5013          & 0.5157   & 0.5106          \\
                               & 1.00E-03             & 0.8673   & 0.8693          & 0.8807          & 0.5106   & 0.8804          \\
                               & 1.00E-04             & 0.9102   & \textbf{0.9240} & 0.9167          & 0.9209   & 0.9151          \\
                               & 1.00E-05             & 0.8758   & 0.8989          & 0.8944          & 0.8793   & 0.8931          \\ \bottomrule 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{SIIM-ISIC Melanoma, MobileNet V3 small}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04 & 1.00E-05        & 1.00E-06        & 0               \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 0.8868   & 0.9275   & 0.9349          & 0.9321          & 0.9293          \\
                               & 1.00E-02             & 0.9338   & 0.9330   & 0.9335          & \textbf{0.9354} & 0.9307          \\
                               & 1.00E-03             & 0.9017   & 0.8944   & 0.8966          & 0.8968          & 0.8993          \\
                               & 1.00E-04             & 0.8333   & 0.8487   & 0.8409          & 0.8531          & 0.8439          \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 0.8962   & 0.9312   & 0.9278          & 0.9299          & \textbf{0.9393} \\
                               & 1.00E-02             & 0.9321   & 0.9347   & 0.9271          & 0.9296          & 0.9332          \\
                               & 1.00E-03             & 0.8999   & 0.8990   & 0.8966          & 0.8994          & 0.8991          \\
                               & 1.00E-04             & 0.8513   & 0.8471   & 0.8479          & 0.8384          & 0.8547          \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 0.8944   & 0.9143   & 0.9042          & 0.9146          & 0.9078          \\
                               & 1.00E-03             & 0.9080   & 0.9418   & \textbf{0.9455} & 0.9452          & 0.9440          \\
                               & 1.00E-04             & 0.8664   & 0.9372   & 0.9326          & 0.9308          & 0.9302          \\
                               & 1.00E-05             & 0.8526   & 0.8938   & 0.8961          & 0.8905          & 0.8896          \\ \bottomrule
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{SIIM-ISIC Melanoma, VGG-13 BN}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04 & 1.00E-05        & 1.00E-06        & 0      \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 0.8774   & 0.8822   & 0.8829          & 0.0000          & 0.8831 \\
                               & 1.00E-02             & 0.9333   & 0.9296   & 0.9342          & \textbf{0.9343} & 0.9331 \\
                               & 1.00E-03             & 0.9143   & 0.9126   & 0.9138          & 0.9160          & 0.9136 \\
                               & 1.00E-04             & 0.8781   & 0.8768   & 0.8758          & 0.8767          & 0.8742 \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 0.8869   & 0.8921   & 0.8912          & 0.8832          & 0.8798 \\
                               & 1.00E-02             & 0.9349   & 0.9362   & \textbf{0.9364} & 0.9342          & 0.9362 \\
                               & 1.00E-03             & 0.9116   & 0.9148   & 0.9132          & 0.9149          & 0.9154 \\
                               & 1.00E-04             & 0.8738   & 0.8734   & 0.8773          & 0.8772          & 0.8760 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 0.8736   & 0.5407   & 0.5053          & 0.5141          & 0.5198 \\
                               & 1.00E-03             & 0.8896   & 0.8997   & 0.9040          & 0.8950          & 0.9066 \\
                               & 1.00E-04             & 0.9357   & 0.9390   & \textbf{0.9421} & 0.9418          & 0.9400 \\
                               & 1.00E-05             & 0.9346   & 0.9240   & 0.9234          & 0.9246          & 0.9248 \\ \bottomrule
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{SIIM-ISIC Melanoma, DeiT-tiny}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04 & 1.00E-05        & 1.00E-06        & 0               \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 0.7999   & 0.0000   & 0.7918          & 0.0000          & 0.8127          \\
                               & 1.00E-02             & 0.9400   & 0.9381   & 0.9381          & 0.9367          & \textbf{0.9406} \\
                               & 1.00E-03             & 0.9354   & 0.9386   & 0.9368          & 0.9355          & 0.9328          \\
                               & 1.00E-04             & 0.8928   & 0.8881   & 0.8966          & 0.8927          & 0.8945          \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 0.8150   & 0.0000   & 0.7920          & 0.7564          & 0.0000          \\
                               & 1.00E-02             & 0.9293   & 0.9328   & \textbf{0.9392} & 0.9349          & 0.9356          \\
                               & 1.00E-03             & 0.9374   & 0.9348   & 0.9372          & 0.9346          & 0.9349          \\
                               & 1.00E-04             & 0.8899   & 0.8940   & 0.8944          & 0.8933          & 0.8919          \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 0.8610   & 0.8221   & 0.8202          & 0.8174          & 0.7964          \\
                               & 1.00E-03             & 0.8851   & 0.8991   & 0.8931          & 0.8933          & 0.8937          \\
                               & 1.00E-04             & 0.8592   & 0.9360   & 0.9336          & \textbf{0.9389} & 0.9364          \\
                               & 1.00E-05             & 0.8112   & 0.9102   & 0.9277          & 0.9164          & 0.9256          \\ \bottomrule 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{SIIM-ISIC Melanoma, ResNet-50}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03        & 1.00E-04 & 1.00E-05        & 1.00E-06        & 0      \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 0.8516          & 0.8495   & 0.8616          & 0.8002          & 0.8375 \\
                               & 1.00E-02             & 0.9279          & 0.9288   & 0.9244          & \textbf{0.9303} & 0.9295 \\
                               & 1.00E-03             & 0.9198          & 0.9141   & 0.9156          & 0.9172          & 0.9162 \\
                               & 1.00E-04             & 0.8668          & 0.8678   & 0.8607          & 0.8701          & 0.8687 \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 0.8736          & 0.8416   & 0.8537          & 0.8530          & 0.8364 \\
                               & 1.00E-02             & 0.9270          & 0.9229   & \textbf{0.9311} & 0.9253          & 0.9293 \\
                               & 1.00E-03             & 0.9179          & 0.9164   & 0.9170          & 0.9198          & 0.9154 \\
                               & 1.00E-04             & 0.8689          & 0.8676   & 0.8645          & 0.8659          & 0.8545 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 0.8643          & 0.8717   & 0.8729          & 0.8733          & 0.8694 \\
                               & 1.00E-03             & 0.8853          & 0.8934   & 0.8921          & 0.9018          & 0.8952 \\
                               & 1.00E-04             & \textbf{0.9297} & 0.9259   & 0.9288          & 0.9238          & 0.9278 \\
                               & 1.00E-05             & 0.8992          & 0.9227   & 0.9218          & 0.9216          & 0.9242 \\ \bottomrule 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{SIIM-ISIC Melanoma, ResNet-152}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03        & 1.00E-04 & 1.00E-05        & 1.00E-06 & 0               \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 0.8652          & 0.8508   & 0.8428          & 0.8532   & 0.8414          \\
                               & 1.00E-02             & 0.9309          & 0.9306   & \textbf{0.9336} & 0.9301   & 0.9312          \\
                               & 1.00E-03             & 0.9159          & 0.9216   & 0.9201          & 0.9199   & 0.9192          \\
                               & 1.00E-04             & 0.8698          & 0.8658   & 0.8721          & 0.8678   & 0.8535          \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 0.8715          & 0.8461   & 0.8579          & 0.8666   & 0.8445          \\
                               & 1.00E-02             & 0.9303          & 0.9277   & 0.9332          & 0.9300   & \textbf{0.9337} \\
                               & 1.00E-03             & 0.9209          & 0.9195   & 0.9210          & 0.9201   & 0.9223          \\
                               & 1.00E-04             & 0.8722          & 0.8761   & 0.8691          & 0.8699   & 0.8639          \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 0.8640          & 0.8540   & 0.8668          & 0.8721   & 0.8775          \\
                               & 1.00E-03             & 0.8820          & 0.8988   & 0.8980          & 0.8946   & 0.8940          \\
                               & 1.00E-04             & \textbf{0.9291} & 0.9271   & \textbf{0.9291} & 0.9277   & 0.9268          \\
                               & 1.00E-05             & 0.9043          & 0.9149   & 0.9168          & 0.9195   & 0.9204          \\ \bottomrule 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{SIIM-ISIC Melanoma, DeiT-small}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03        & 1.00E-04 & 1.00E-05        & 1.00E-06        & 0      \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 0.0000          & 0.0000   & 0.8113          & 0.0000          & 0.0000 \\
                               & 1.00E-02             & 0.9440          & 0.9426   & \textbf{0.9451} & 0.9407          & 0.9439 \\
                               & 1.00E-03             & 0.9372          & 0.9350   & 0.9336          & 0.9346          & 0.9282 \\
                               & 1.00E-04             & 0.8902          & 0.8798   & 0.8802          & 0.8833          & 0.8693 \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 0.0000          & 0.0000   & 0.0000          & 0.0000          & 0.6260 \\
                               & 1.00E-02             & \textbf{0.9440} & 0.9433   & 0.9355          & 0.9391          & 0.9438 \\
                               & 1.00E-03             & 0.9365          & 0.9341   & 0.9309          & 0.9344          & 0.9300 \\
                               & 1.00E-04             & 0.8822          & 0.8874   & 0.8791          & 0.8905          & 0.8850 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 0.8707          & 0.8276   & 0.8058          & 0.8107          & 0.8055 \\
                               & 1.00E-03             & 0.8889          & 0.8955   & 0.8912          & 0.8994          & 0.8973 \\
                               & 1.00E-04             & 0.8694          & 0.9423   & 0.9436          & \textbf{0.9439} & 0.9423 \\
                               & 1.00E-05             & 0.8242          & 0.9208   & 0.9370          & 0.9395          & 0.9348 \\ \bottomrule 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{SIIM-ISIC Melanoma, PNASNet-5 large}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04        & 1.00E-05 & 1.00E-06        & 0      \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 0.9040   & \textbf{0.9441} & 0.9426   & 0.9395          & 0.9373 \\
                               & 1.00E-02             & 0.9341   & 0.9310          & 0.9297   & 0.9246          & 0.9297 \\
                               & 1.00E-03             & 0.8969   & 0.8908          & 0.8935   & 0.8959          & 0.8948 \\
                               & 1.00E-04             & 0.8280   & 0.8272          & 0.8263   & 0.8253          & 0.8319 \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 0.9126   & 0.9445          & 0.9393   & \textbf{0.9449} & 0.9365 \\
                               & 1.00E-02             & 0.9316   & 0.9330          & 0.9316   & 0.9320          & 0.9290 \\
                               & 1.00E-03             & 0.8933   & 0.8934          & 0.8928   & 0.8904          & 0.8918 \\
                               & 1.00E-04             & 0.8265   & 0.8242          & 0.8213   & 0.8289          & 0.8250 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 0.8770   & 0.8818          & 0.8713   & 0.8715          & 0.8744 \\
                               & 1.00E-03             & 0.9139   & 0.9300          & 0.9375   & \textbf{0.9392} & 0.9323 \\
                               & 1.00E-04             & 0.9195   & 0.9365          & 0.9366   & 0.9340          & 0.9336 \\
                               & 1.00E-05             & 0.8836   & 0.9214          & 0.9166   & 0.9164          & 0.9139 \\ \bottomrule 
\end{tabular}
\end{table}

\clearpage


\subsection{Cassava Leaf Disease}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{Cassava Leaf Disease, AlexNet}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03       & 1.00E-04       & 1.00E-05 & 1.00E-06       & 0     \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 0.00           & 0.00           & 0.00     & 0.00           & 0.00  \\
                               & 1.00E-02             & 0.00           & 0.00           & 61.50    & 0.00           & 0.00  \\
                               & 1.00E-03             & 80.93          & \textbf{81.50} & 81.31    & 81.29          & 80.91 \\
                               & 1.00E-04             & 76.85          & 77.03          & 77.29    & 77.22          & 76.89 \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 0.00           & 0.00           & 0.00     & 0.00           & 0.00  \\
                               & 1.00E-02             & 0.00           & 0.00           & 0.00     & 0.00           & 0.00  \\
                               & 1.00E-03             & 81.21          & 81.21          & 81.12    & \textbf{81.38} & 81.29 \\
                               & 1.00E-04             & 77.24          & 77.55          & 77.36    & 76.78          & 77.31 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 61.50          & 61.50          & 61.50    & 61.50          & 61.50 \\
                               & 1.00E-03             & 79.84          & 61.50          & 79.30    & 61.50          & 61.50 \\
                               & 1.00E-04             & \textbf{82.48} & 79.98          & 79.67    & 79.77          & 79.39 \\
                               & 1.00E-05             & 73.32          & 79.39          & 79.44    & 78.88          & 78.69 \\ \bottomrule 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{Cassava Leaf Disease, MobileNet V3 small}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03       & 1.00E-04       & 1.00E-05 & 1.00E-06 & 0     \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 84.45          & \textbf{85.27} & 84.99    & 84.90    & 84.90 \\
                               & 1.00E-02             & 84.69          & 84.45          & 84.62    & 84.57    & 84.57 \\
                               & 1.00E-03             & 84.10          & 83.94          & 83.63    & 83.63    & 83.77 \\
                               & 1.00E-04             & 73.25          & 72.64          & 73.11    & 73.07    & 72.50 \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & \textbf{85.13} & 84.43          & 84.01    & 84.45    & 84.12 \\
                               & 1.00E-02             & 84.52          & 84.01          & 84.36    & 84.05    & 84.31 \\
                               & 1.00E-03             & 84.01          & 83.68          & 83.91    & 83.80    & 84.05 \\
                               & 1.00E-04             & 73.14          & 72.97          & 73.14    & 72.64    & 73.28 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & \textbf{85.81} & 85.62          & 85.29    & 85.34    & 85.71 \\
                               & 1.00E-03             & 84.80          & 83.56          & 84.17    & 84.12    & 84.15 \\
                               & 1.00E-04             & 68.86          & 84.78          & 84.48    & 84.43    & 84.76 \\
                               & 1.00E-05             & 62.03          & 80.80          & 81.65    & 81.23    & 80.92 \\ \bottomrule
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{Cassava Leaf Disease, VGG-13 BN}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03       & 1.00E-04       & 1.00E-05       & 1.00E-06 & 0     \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 87.48          & 87.80          & \textbf{88.48} & 87.90    & 88.06 \\
                               & 1.00E-02             & 86.89          & 87.27          & 87.06          & 87.41    & 86.82 \\
                               & 1.00E-03             & 86.94          & 86.94          & 86.89          & 86.96    & 86.78 \\
                               & 1.00E-04             & 81.40          & 81.73          & 81.85          & 81.52    & 81.75 \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & \textbf{88.25} & 87.71          & 87.62          & 87.36    & 87.78 \\
                               & 1.00E-02             & 86.80          & 87.29          & 86.92          & 86.50    & 87.03 \\
                               & 1.00E-03             & 86.96          & 87.22          & 86.85          & 86.64    & 87.06 \\
                               & 1.00E-04             & 81.61          & 81.73          & 81.12          & 81.26    & 81.45 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 61.50          & 61.50          & 61.50          & 61.50    & 76.17 \\
                               & 1.00E-03             & 87.71          & \textbf{87.76} & 87.20          & 87.41    & 87.27 \\
                               & 1.00E-04             & 87.13          & 86.94          & 86.99          & 86.73    & 86.78 \\
                               & 1.00E-05             & 87.17          & 86.68          & 86.50          & 86.73    & 86.21 \\ \bottomrule
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{Cassava Leaf Disease, DeiT-tiny}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04       & 1.00E-05 & 1.00E-06       & 0              \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 61.50    & 61.50          & 61.50    & 61.52          & 63.08          \\
                               & 1.00E-02             & 84.93    & 84.46          & 84.51    & 84.49          & 84.86          \\
                               & 1.00E-03             & 85.86    & 85.49          & 85.56    & \textbf{85.96} & 85.91          \\
                               & 1.00E-04             & 84.18    & 84.21          & 83.53    & 84.14          & 84.21          \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 61.50    & 61.50          & 66.40    & 61.50          & 61.50          \\
                               & 1.00E-02             & 84.44    & 84.44          & 84.21    & 83.88          & 84.35          \\
                               & 1.00E-03             & 85.51    & \textbf{85.82} & 85.37    & 85.21          & 85.63          \\
                               & 1.00E-04             & 83.60    & 83.43          & 84.25    & 83.90          & 83.81          \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 65.93    & 62.69          & 62.66    & 61.52          & 61.61          \\
                               & 1.00E-03             & 78.20    & 81.29          & 81.03    & 80.77          & 80.91          \\
                               & 1.00E-04             & 79.65    & 85.02          & 85.51    & 85.33          & 85.16          \\
                               & 1.00E-05             & 65.49    & 84.37          & 85.42    & 85.58          & \textbf{85.79} \\ \bottomrule 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{Cassava Leaf Disease, ResNet-50}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03       & 1.00E-04       & 1.00E-05 & 1.00E-06 & 0     \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 82.41          & 82.92          & 74.91    & 84.39    & 80.35 \\
                               & 1.00E-02             & 86.36          & \textbf{86.36} & 85.89    & 85.93    & 85.65 \\
                               & 1.00E-03             & 85.82          & 85.65          & 85.82    & 85.58    & 85.93 \\
                               & 1.00E-04             & 78.71          & 78.76          & 78.74    & 79.02    & 78.81 \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 85.09          & 83.83          & 78.83    & 77.78    & 85.16 \\
                               & 1.00E-02             & 85.96          & \textbf{86.10} & 85.61    & 85.65    & 85.82 \\
                               & 1.00E-03             & 85.56          & 85.98          & 85.93    & 86.03    & 85.84 \\
                               & 1.00E-04             & 78.74          & 78.39          & 78.34    & 78.60    & 78.25 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 83.90          & 83.81          & 84.46    & 83.93    & 83.88 \\
                               & 1.00E-03             & \textbf{87.41} & 86.36          & 86.03    & 86.10    & 85.82 \\
                               & 1.00E-04             & 86.64          & 86.40          & 86.29    & 86.19    & 86.47 \\
                               & 1.00E-05             & 84.72          & 86.00          & 85.79    & 86.03    & 85.86 \\ \bottomrule 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{Cassava Leaf Disease, ResNet-152}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03       & 1.00E-04       & 1.00E-05 & 1.00E-06 & 0     \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 81.29          & 81.24          & 73.01    & 77.08    & 74.77 \\
                               & 1.00E-02             & 85.35          & \textbf{86.12} & 85.44    & 85.82    & 85.19 \\
                               & 1.00E-03             & 85.56          & 85.37          & 84.98    & 85.40    & 85.16 \\
                               & 1.00E-04             & 78.62          & 78.86          & 78.90    & 78.86    & 78.57 \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 82.17          & 76.71          & 79.44    & 76.99    & 77.22 \\
                               & 1.00E-02             & \textbf{86.10} & 85.54          & 86.03    & 85.70    & 85.75 \\
                               & 1.00E-03             & 85.58          & 85.21          & 85.37    & 85.23    & 85.54 \\
                               & 1.00E-04             & 79.46          & 79.14          & 78.74    & 78.74    & 79.04 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 83.71          & 85.02          & 82.01    & 83.15    & 83.95 \\
                               & 1.00E-03             & \textbf{86.68} & 86.36          & 86.19    & 86.19    & 85.86 \\
                               & 1.00E-04             & 86.21          & 86.59          & 86.10    & 86.29    & 85.61 \\
                               & 1.00E-05             & 83.57          & 85.05          & 85.09    & 85.19    & 85.68 \\ \bottomrule
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{Cassava Leaf Disease, DeiT-small}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04 & 1.00E-05       & 1.00E-06 & 0              \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 0.00     & 0.00     & 61.50          & 61.50    & 0.00           \\
                               & 1.00E-02             & 85.26    & 85.51    & 85.19          & 85.35    & 85.00          \\
                               & 1.00E-03             & 85.98    & 86.64    & 86.61          & 86.75    & \textbf{87.06} \\
                               & 1.00E-04             & 84.11    & 83.88    & 83.88          & 84.37    & 84.07          \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 61.52    & 0.00     & 61.50          & 0.00     & 64.21          \\
                               & 1.00E-02             & 85.56    & 85.23    & 85.30          & 85.42    & 85.21          \\
                               & 1.00E-03             & 86.50    & 86.19    & \textbf{86.68} & 86.29    & 86.21          \\
                               & 1.00E-04             & 83.95    & 84.02    & 84.18          & 84.00    & 84.09          \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 65.14    & 63.13    & 61.75          & 62.24    & 62.52          \\
                               & 1.00E-03             & 78.53    & 80.14    & 79.49          & 80.61    & 80.44          \\
                               & 1.00E-04             & 82.71    & 85.61    & 86.26          & 86.64    & 86.26          \\
                               & 1.00E-05             & 69.56    & 85.89    & \textbf{86.66} & 86.59    & 86.40          \\ \bottomrule
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{Cassava Leaf Disease, PNASNet-5 large}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03       & 1.00E-04       & 1.00E-05       & 1.00E-06 & 0     \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & \textbf{86.87} & 85.84          & 86.50          & 86.14    & 86.14 \\
                               & 1.00E-02             & 85.61          & 84.46          & 83.79          & 84.32    & 84.77 \\
                               & 1.00E-03             & 82.83          & 82.55          & 82.92          & 82.59    & 82.87 \\
                               & 1.00E-04             & 74.25          & 74.65          & 74.16          & 74.74    & 73.76 \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 85.79          & \textbf{86.68} & 86.59          & 86.38    & 86.64 \\
                               & 1.00E-02             & 84.81          & 85.12          & 85.02          & 84.84    & 84.49 \\
                               & 1.00E-03             & 82.29          & 82.45          & 82.59          & 82.92    & 82.45 \\
                               & 1.00E-04             & 74.37          & 74.56          & 74.04          & 74.07    & 74.35 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 86.14          & 83.95          & \textbf{86.59} & 85.26    & 84.39 \\
                               & 1.00E-03             & 85.70          & 86.00          & 86.45          & 85.79    & 86.31 \\
                               & 1.00E-04             & 84.02          & 86.00          & 86.17          & 86.29    & 85.65 \\
                               & 1.00E-05             & 80.65          & 83.53          & 83.06          & 82.69    & 82.76 \\ \bottomrule 
\end{tabular}
\end{table}

\clearpage

\subsection{EuroSAT}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{EuroSAT, AlexNet}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03       & 1.00E-04       & 1.00E-05 & 1.00E-06       & 0     \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 0.00           & 0.00           & 0.00     & 0.00           & 0.00  \\
                               & 1.00E-02             & 97.13          & \textbf{97.69} & 0.00     & 11.11          & 97.04 \\
                               & 1.00E-03             & 97.56          & 97.33          & 97.59    & 97.28          & 97.48 \\
                               & 1.00E-04             & 94.43          & 94.76          & 94.48    & 94.72          & 94.65 \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 0.00           & 0.00           & 0.00     & 0.00           & 0.00  \\
                               & 1.00E-02             & \textbf{97.74} & 97.65          & 0.00     & 0.00           & 11.11 \\
                               & 1.00E-03             & 97.46          & 97.37          & 97.43    & 97.26          & 97.43 \\
                               & 1.00E-04             & 94.69          & 94.63          & 94.63    & 94.65          & 94.56 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 11.63          & 11.11          & 11.11    & 11.11          & 11.11 \\
                               & 1.00E-03             & 97.04          & 97.39          & 97.13    & 96.87          & 97.35 \\
                               & 1.00E-04             & 96.33          & \textbf{97.93} & 97.81    & \textbf{97.93} & 97.80 \\
                               & 1.00E-05             & 88.52          & 95.96          & 96.15    & 96.13          & 96.22 \\ \bottomrule 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{EuroSAT, MobileNet V3 small}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04       & 1.00E-05 & 1.00E-06       & 0     \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 96.91    & 98.74          & 98.61    & 98.67          & 98.52 \\
                               & 1.00E-02             & 98.91    & \textbf{99.00} & 98.85    & 98.83          & 98.76 \\
                               & 1.00E-03             & 97.70    & 97.74          & 97.57    & 97.39          & 97.35 \\
                               & 1.00E-04             & 92.41    & 92.70          & 92.69    & 92.28          & 92.80 \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 97.50    & 98.70          & 98.76    & \textbf{99.00} & 98.76 \\
                               & 1.00E-02             & 98.91    & 98.94          & 98.89    & 98.76          & 98.70 \\
                               & 1.00E-03             & 97.54    & 97.48          & 97.54    & 97.54          & 97.43 \\
                               & 1.00E-04             & 92.13    & 92.43          & 92.43    & 92.80          & 92.54 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 97.67    & 98.31          & 98.61    & 98.46          & 98.72 \\
                               & 1.00E-03             & 96.85    & \textbf{99.15} & 99.00    & \textbf{99.15} & 99.11 \\
                               & 1.00E-04             & 78.94    & 98.96          & 98.81    & 98.65          & 98.59 \\
                               & 1.00E-05             & 19.11    & 96.65          & 96.54    & 96.39          & 96.41 \\ \bottomrule 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{EuroSAT, VGG-13 BN}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03       & 1.00E-04 & 1.00E-05       & 1.00E-06 & 0              \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 97.56          & 97.74    & 97.43          & 97.89    & 97.56          \\
                               & 1.00E-02             & 98.67          & 98.70    & \textbf{98.83} & 98.50    & 98.54          \\
                               & 1.00E-03             & 98.24          & 98.07    & 98.26          & 98.24    & 98.20          \\
                               & 1.00E-04             & 96.11          & 96.00    & 95.69          & 95.96    & 95.98          \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 97.96          & 97.89    & 97.85          & 97.81    & 97.65          \\
                               & 1.00E-02             & 98.69          & 98.63    & 98.70          & 98.63    & \textbf{98.85} \\
                               & 1.00E-03             & 98.11          & 98.11    & 98.07          & 98.19    & 98.13          \\
                               & 1.00E-04             & 96.07          & 95.91    & 95.94          & 96.24    & 96.06          \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 95.67          & 85.52    & 84.61          & 55.81    & 90.80          \\
                               & 1.00E-03             & 98.17          & 98.24    & 98.11          & 98.30    & 98.19          \\
                               & 1.00E-04             & \textbf{98.65} & 98.61    & 98.59          & 98.54    & 98.54          \\
                               & 1.00E-05             & 98.07          & 98.02    & 98.06          & 97.94    & 97.87          \\ \bottomrule 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{EuroSAT, DeiT-tiny}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03       & 1.00E-04 & 1.00E-05       & 1.00E-06 & 0     \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 0.00           & 33.15    & 22.24          & 24.13    & 28.67 \\
                               & 1.00E-02             & 98.80          & 98.93    & 98.78          & 98.87    & 98.87 \\
                               & 1.00E-03             & 98.81          & 98.89    & \textbf{98.96} & 98.91    & 98.91 \\
                               & 1.00E-04             & 98.04          & 97.80    & 97.91          & 97.89    & 97.70 \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 11.15          & 18.28    & 96.24          & 58.72    & 43.87 \\
                               & 1.00E-02             & \textbf{99.07} & 98.85    & 98.98          & 98.94    & 98.91 \\
                               & 1.00E-03             & 98.93          & 98.72    & 98.98          & 98.94    & 98.89 \\
                               & 1.00E-04             & 97.74          & 97.69    & 97.76          & 97.78    & 97.89 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 93.70          & 66.96    & 49.85          & 56.09    & 49.44 \\
                               & 1.00E-03             & 96.26          & 98.24    & 97.98          & 97.87    & 98.04 \\
                               & 1.00E-04             & 95.69          & 98.94    & \textbf{99.11} & 99.02    & 99.04 \\
                               & 1.00E-05             & 78.91          & 97.98    & 98.50          & 98.57    & 98.69 \\ \bottomrule
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{EuroSAT, ResNet-50}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03       & 1.00E-04 & 1.00E-05 & 1.00E-06       & 0     \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 95.43          & 93.96    & 96.57    & 94.59          & 95.43 \\
                               & 1.00E-02             & \textbf{99.13} & 98.85    & 98.69    & 98.81          & 98.85 \\
                               & 1.00E-03             & 98.72          & 98.80    & 98.59    & 98.63          & 98.57 \\
                               & 1.00E-04             & 96.83          & 96.69    & 96.63    & 96.72          & 96.85 \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 96.61          & 93.76    & 94.00    & 87.26          & 94.54 \\
                               & 1.00E-02             & \textbf{99.04} & 98.87    & 98.94    & 98.80          & 98.87 \\
                               & 1.00E-03             & 98.67          & 98.56    & 98.57    & 98.65          & 98.50 \\
                               & 1.00E-04             & 96.63          & 96.39    & 96.74    & 96.74          & 96.56 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 96.93          & 96.83    & 96.81    & 95.37          & 96.67 \\
                               & 1.00E-03             & 98.56          & 98.54    & 98.43    & 98.57          & 98.54 \\
                               & 1.00E-04             & 98.63          & 99.09    & 99.06    & \textbf{99.19} & 99.07 \\
                               & 1.00E-05             & 97.89          & 98.76    & 98.57    & 98.57          & 98.67 \\ \bottomrule
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{EuroSAT, ResNet-152}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03       & 1.00E-04 & 1.00E-05 & 1.00E-06       & 0     \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 96.54          & 96.28    & 93.61    & 95.94          & 89.37 \\
                               & 1.00E-02             & \textbf{99.02} & 98.96    & 98.96    & 98.69          & 98.96 \\
                               & 1.00E-03             & 98.72          & 98.61    & 98.63    & 98.54          & 98.80 \\
                               & 1.00E-04             & 96.78          & 96.78    & 96.70    & 97.02          & 96.76 \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 96.87          & 90.63    & 96.28    & 93.87          & 94.35 \\
                               & 1.00E-02             & \textbf{99.02} & 98.91    & 98.85    & 98.74          & 99.00 \\
                               & 1.00E-03             & 98.44          & 98.43    & 98.57    & 98.54          & 98.43 \\
                               & 1.00E-04             & 96.35          & 96.50    & 96.37    & 96.26          & 96.65 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 96.48          & 96.30    & 96.80    & 96.54          & 96.70 \\
                               & 1.00E-03             & 98.50          & 98.48    & 98.57    & 98.59          & 98.54 \\
                               & 1.00E-04             & 98.50          & 99.09    & 99.00    & \textbf{99.15} & 99.09 \\
                               & 1.00E-05             & 97.35          & 98.70    & 98.69    & 98.44          & 98.56 \\ \bottomrule 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{EuroSAT, DeiT-small}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04 & 1.00E-05       & 1.00E-06       & 0              \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 0.00     & 40.61    & 38.22          & 24.39          & 32.80          \\
                               & 1.00E-02             & 99.00    & 99.04    & 99.04          & \textbf{99.06} & \textbf{99.06} \\
                               & 1.00E-03             & 99.00    & 98.91    & 98.96          & 98.93          & 98.87          \\
                               & 1.00E-04             & 97.76    & 97.33    & 97.74          & 97.52          & 97.91          \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 0.00     & 0.00     & 0.00           & 10.22          & 0.00           \\
                               & 1.00E-02             & 99.06    & 99.15    & \textbf{99.20} & 99.02          & 99.04          \\
                               & 1.00E-03             & 98.96    & 98.96    & 98.93          & 99.06          & 98.96          \\
                               & 1.00E-04             & 97.56    & 97.56    & 97.59          & 97.69          & 97.46          \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 89.28    & 57.61    & 46.48          & 51.43          & 44.85          \\
                               & 1.00E-03             & 96.61    & 98.15    & 98.28          & 98.13          & 98.41          \\
                               & 1.00E-04             & 95.76    & 99.13    & 99.11          & \textbf{99.17} & 99.15          \\
                               & 1.00E-05             & 90.30    & 98.69    & 98.87          & 98.76          & 99.02          \\ \bottomrule 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{EuroSAT, PNASNet-5 large}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03       & 1.00E-04       & 1.00E-05       & 1.00E-06 & 0     \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 98.41          & 98.78          & 98.76          & 98.50    & 98.74 \\
                               & 1.00E-02             & \textbf{98.85} & \textbf{98.85} & 98.81          & 98.81    & 98.80 \\
                               & 1.00E-03             & 98.09          & 98.04          & 98.07          & 98.02    & 97.96 \\
                               & 1.00E-04             & 95.26          & 95.11          & 95.37          & 95.33    & 95.65 \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 98.46          & 99.07          & \textbf{99.13} & 99.00    & 99.09 \\
                               & 1.00E-02             & 98.89          & 98.93          & 98.69          & 98.80    & 98.65 \\
                               & 1.00E-03             & 98.00          & 97.94          & 97.96          & 97.98    & 97.98 \\
                               & 1.00E-04             & 95.28          & 95.15          & 95.30          & 95.41    & 95.41 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 97.83          & 97.20          & 97.44          & 96.74    & 97.78 \\
                               & 1.00E-03             & 98.54          & 98.94          & 98.96          & 98.65    & 98.80 \\
                               & 1.00E-04             & 98.67          & 99.04          & \textbf{99.17} & 99.02    & 99.13 \\
                               & 1.00E-05             & 96.85          & 98.63          & 98.69          & 98.46    & 98.52 \\ \bottomrule 
\end{tabular}
\end{table}

\begin{table}[h]
\centering
\caption{CIFAR-10, AlexNet}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04 & 1.00E-05       & 1.00E-06       & 0     \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 10.00    & 10.00    & 10.00          & 10.00          & 10.00 \\
                               & 1.00E-02             & 93.06    & 93.29    & 93.12          & \textbf{93.41} & 93.30 \\
                               & 1.00E-03             & 92.45    & 92.60    & 92.53          & 92.47          & 92.69 \\
                               & 1.00E-04             & 88.31    & 88.14    & 88.20          & 88.03          & 88.33 \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 10.00    & 10.00    & 10.00          & 10.00          & 10.00 \\
                               & 1.00E-02             & 93.37    & 93.45    & \textbf{93.56} & 93.48          & 93.41 \\
                               & 1.00E-03             & 92.72    & 92.73    & 92.57          & 92.80          & 92.72 \\
                               & 1.00E-04             & 88.29    & 88.39    & 88.27          & 88.38          & 88.24 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 10.00    & 10.00    & 10.00          & 10.00          & 10.00 \\
                               & 1.00E-03             & 89.31    & 89.65    & 89.43          & 87.78          & 86.64 \\
                               & 1.00E-04             & 84.60    & 93.49    & \textbf{93.96} & 93.95          & 93.78 \\
                               & 1.00E-05             & 75.43    & 88.13    & 91.37          & 91.56          & 91.62 \\ \bottomrule
\end{tabular}
\end{table}

\begin{table}[h]
\centering
\caption{CIFAR-10, MobileNet V3 small}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04       & 1.00E-05       & 1.00E-06       & 0     \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 89.43    & 95.83          & 95.94          & 95.83          & 95.90 \\
                               & 1.00E-02             & 95.45    & \textbf{96.06} & 95.96          & 95.94          & 96.00 \\
                               & 1.00E-03             & 94.48    & 94.41          & 94.25          & 94.37          & 94.49 \\
                               & 1.00E-04             & 87.25    & 87.05          & 87.56          & 87.44          & 87.04 \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 90.95    & 95.82          & \textbf{96.30} & 95.97          & 95.91 \\
                               & 1.00E-02             & 95.09    & 96.05          & 95.96          & 96.22          & 95.95 \\
                               & 1.00E-03             & 94.31    & 94.33          & 94.49          & 94.34          & 94.35 \\
                               & 1.00E-04             & 87.28    & 87.31          & 87.33          & 87.37          & 87.26 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 90.60    & 93.99          & 93.52          & 93.52          & 93.90 \\
                               & 1.00E-03             & 77.57    & 96.02          & \textbf{96.43} & \textbf{96.43} & 96.33 \\
                               & 1.00E-04             & 19.36    & 94.41          & 95.57          & 95.52          & 95.41 \\
                               & 1.00E-05             & 10.44    & 86.22          & 92.39          & 92.26          & 92.20 \\ \bottomrule
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{CIFAR-10, VGG-13 BN}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03       & 1.00E-04       & 1.00E-05 & 1.00E-06 & 0     \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 92.99          & 94.48          & 94.16    & 94.39    & 94.70 \\
                               & 1.00E-02             & \textbf{95.60} & 95.51          & 95.54    & 95.42    & 95.54 \\
                               & 1.00E-03             & 94.21          & 94.14          & 94.24    & 94.14    & 94.04 \\
                               & 1.00E-04             & 89.02          & 89.18          & 89.09    & 89.05    & 89.04 \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 94.38          & 95.15          & 95.09    & 95.14    & 94.80 \\
                               & 1.00E-02             & \textbf{95.73} & 95.56          & 95.45    & 95.44    & 95.58 \\
                               & 1.00E-03             & 94.08          & 94.26          & 94.11    & 94.27    & 94.15 \\
                               & 1.00E-04             & 89.06          & 89.14          & 89.18    & 89.20    & 89.12 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 10.00          & 10.00          & 10.00    & 65.71    & 10.00 \\
                               & 1.00E-03             & 94.07          & 94.42          & 94.30    & 94.37    & 94.49 \\
                               & 1.00E-04             & 93.15          & \textbf{95.59} & 95.35    & 95.32    & 95.24 \\
                               & 1.00E-05             & 87.49          & 93.51          & 93.12    & 92.93    & 93.09 \\ \bottomrule 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{CIFAR-10, DeiT-tiny}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04       & 1.00E-05       & 1.00E-06 & 0     \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 41.05    & 14.61          & 15.15          & 0.00     & 25.24 \\
                               & 1.00E-02             & 95.64    & 96.65          & 96.70          & 96.48    & 96.66 \\
                               & 1.00E-03             & 96.97    & \textbf{97.05} & 96.91          & 96.74    & 96.96 \\
                               & 1.00E-04             & 95.59    & 95.69          & 95.71          & 95.66    & 95.77 \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 52.88    & 71.15          & 71.15          & 10.51    & 19.44 \\
                               & 1.00E-02             & 95.62    & 96.90          & 96.89          & 96.73    & 96.80 \\
                               & 1.00E-03             & 97.00    & 96.86          & \textbf{97.13} & 96.95    & 96.81 \\
                               & 1.00E-04             & 95.65    & 95.65          & 95.50          & 95.65    & 95.56 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 75.08    & 30.32          & 27.17          & 25.22    & 25.08 \\
                               & 1.00E-03             & 73.62    & 91.17          & 90.75          & 92.00    & 88.31 \\
                               & 1.00E-04             & 83.80    & 95.45          & \textbf{97.21} & 97.02    & 97.12 \\
                               & 1.00E-05             & 51.23    & 93.25          & 96.25          & 96.16    & 96.38 \\ \bottomrule 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{CIFAR-10, ResNet-50}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04       & 1.00E-05       & 1.00E-06       & 0     \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 89.29    & 88.88          & 89.11          & 83.66          & 82.10 \\
                               & 1.00E-02             & 97.26    & 97.16          & 97.24          & \textbf{97.33} & 97.27 \\
                               & 1.00E-03             & 96.76    & 96.93          & 96.83          & 96.82          & 96.90 \\
                               & 1.00E-04             & 94.76    & 94.70          & 94.55          & 94.62          & 94.59 \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 93.00    & 89.38          & 89.23          & 91.43          & 89.63 \\
                               & 1.00E-02             & 97.48    & 97.44          & \textbf{97.61} & 97.34          & 97.46 \\
                               & 1.00E-03             & 96.98    & 96.79          & 96.86          & 96.74          & 96.84 \\
                               & 1.00E-04             & 94.54    & 94.60          & 94.60          & 94.60          & 94.67 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 90.26    & 91.89          & 86.66          & 89.87          & 91.33 \\
                               & 1.00E-03             & 95.02    & 95.77          & 95.88          & 95.74          & 96.11 \\
                               & 1.00E-04             & 94.12    & \textbf{97.47} & 97.27          & 97.42          & 97.35 \\
                               & 1.00E-05             & 93.77    & 96.94          & 96.90          & 96.73          & 96.72 \\ \bottomrule 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{CIFAR-10, ResNet-152}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03       & 1.00E-04 & 1.00E-05 & 1.00E-06 & 0              \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 88.38          & 83.69    & 81.18    & 81.74    & 79.01          \\
                               & 1.00E-02             & 97.80          & 97.83    & 97.81    & 97.73    & 97.87          \\
                               & 1.00E-03             & 97.64          & 97.70    & 97.79    & 97.66    & \textbf{97.91} \\
                               & 1.00E-04             & 96.07          & 96.08    & 96.18    & 96.30    & 96.28          \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 90.93          & 86.12    & 81.09    & 86.21    & 78.29          \\
                               & 1.00E-02             & \textbf{98.29} & 97.93    & 97.96    & 98.09    & 98.09          \\
                               & 1.00E-03             & 97.73          & 97.67    & 97.72    & 97.62    & 97.64          \\
                               & 1.00E-04             & 96.28          & 96.12    & 96.04    & 95.99    & 96.14          \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 91.41          & 88.18    & 87.34    & 88.64    & 90.55          \\
                               & 1.00E-03             & 94.64          & 95.68    & 95.03    & 95.40    & 94.95          \\
                               & 1.00E-04             & 94.56          & 97.63    & 97.55    & 97.67    & \textbf{97.79} \\
                               & 1.00E-05             & 93.13          & 97.39    & 97.59    & 97.52    & 97.36          \\ \bottomrule
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{CIFAR-10, DeiT-small}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03       & 1.00E-04       & 1.00E-05       & 1.00E-06       & 0     \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 0.00           & 10.62          & 0.00           & 0.00           & 0.00  \\
                               & 1.00E-02             & 96.71          & 97.89          & 97.85          & 97.77          & 97.82 \\
                               & 1.00E-03             & \textbf{98.02} & 98.00          & 97.97          & 97.93          & 97.95 \\
                               & 1.00E-04             & 97.26          & 97.01          & 97.09          & 97.10          & 97.19 \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 14.57          & 80.13          & 0.00           & 0.00           & 0.00  \\
                               & 1.00E-02             & 96.59          & \textbf{98.13} & \textbf{98.13} & 98.00          & 98.06 \\
                               & 1.00E-03             & 97.95          & 97.97          & 97.97          & 97.94          & 98.01 \\
                               & 1.00E-04             & 97.16          & 97.15          & 97.27          & 97.12          & 97.15 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 75.17          & 28.72          & 25.95          & 25.06          & 25.62 \\
                               & 1.00E-03             & 82.62          & 88.98          & 87.08          & 90.98          & 86.81 \\
                               & 1.00E-04             & 88.16          & 96.46          & 97.99          & \textbf{98.21} & 98.06 \\
                               & 1.00E-05             & 65.19          & 96.40          & 97.94          & 97.86          & 97.90 \\ \bottomrule 
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{CIFAR-10, PNASNet-5 large}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                               & lr \textbackslash wd & 1.00E-03 & 1.00E-04 & 1.00E-05       & 1.00E-06       & 0     \\ \midrule
\multirow{4}{*}{SGD / Step}    & 1.00E-01             & 94.92    & 97.29    & 97.37          & 97.60          & 97.31 \\
                               & 1.00E-02             & 97.70    & 97.99    & 98.19          & \textbf{98.21} & 98.18 \\
                               & 1.00E-03             & 97.51    & 97.49    & 97.40          & 97.49          & 97.42 \\
                               & 1.00E-04             & 95.10    & 95.21    & 95.09          & 95.10          & 94.97 \\ \midrule
\multirow{4}{*}{SGD / Cosine}  & 1.00E-01             & 95.48    & 97.35    & 97.71          & 97.63          & 97.72 \\
                               & 1.00E-02             & 97.70    & 98.11    & 98.12          & \textbf{98.15} & 98.12 \\
                               & 1.00E-03             & 97.55    & 97.47    & 97.31          & 97.29          & 97.47 \\
                               & 1.00E-04             & 95.06    & 95.10    & 95.06          & 95.10          & 95.14 \\ \midrule
\multirow{4}{*}{Adam / Cosine} & 1.00E-02             & 93.61    & 92.21    & 92.71          & 92.50          & 92.41 \\
                               & 1.00E-03             & 95.14    & 97.09    & 97.20          & 97.05          & 97.25 \\
                               & 1.00E-04             & 95.84    & 97.55    & \textbf{98.21} & 97.97          & 98.17 \\
                               & 1.00E-05             & 93.36    & 97.27    & 97.61          & 97.58          & 97.67 \\ \bottomrule
\end{tabular}
\end{table}

\clearpage



==> setup.tex <==
% !TEX root = imagenet_applications_main.tex
\section{Experiment setup}

\subsection{Models}
\begin{table}[hbt]
\scriptsize
    \centering
    % \rowcolors{2}{}{gray!25}
    \vspace{-0.5em}
  \caption{\label{tab:imagenet_models} We examine the effectiveness of transfer learning from a number of models pretrained on ImageNet, including both CNNs and Vision Transformers.}
  \vspace{-0.5em}
  \centering
    \begin{tabular}{lccc}
    \toprule
    Model                & ImageNet top-1 & \# params & Year Released \\\midrule
    AlexNet~\citep{krizhevskySH12}  & 56.5   & 61M  & 2012 \\
    SqueezeNet 1.1~\citep{IandolaMAHDK16} & 58.2 & 1.2M & 2016 \\
    ShuffleNetV2x0.5~\citep{MaZZS18} & 60.6 & 1.4M & 2018 \\
    MobileNet V3 small~\citep{HowardPALSCWCTC19}   & 67.7   & 2.5M  & 2019 \\
    ShuffleNetV2x1.0~\citep{MaZZS18} & 69.4 & 2.3M & 2018 \\
    VGG-13 BN~\citep{SimonyanZ14a}   & 71.6   & 133M  & 2014/2015 \\
    DeiT-tiny~\citep{TouvronCDMSJ21}     & 72.2   & 5.7M  & 2020 \\
    VGG-16 BN~\citep{SimonyanZ14a} & 73.4 & 138M & 2014/2015 \\
    DenseNet-121~\citep{HuangLMW17} & 74.4 & 8.0M & 2016 \\
    ResNet-50~\citep{HeZRS16}      & 76.1   & 26M  & 2015 \\
    ResNeXt-50-32x4d~\citep{XieGDTH17} & 77.6 & 25M & 2016 \\
    EfficientNet B0~\citep{TanL19} & 77.7 & 5.3M & 2019 \\
    ResNet-152~\citep{HeZRS16}  & 78.3   & 60M  & 2015 \\
    ViT-B/16~\citep{DosovitskiyB0WZ21,SteinerViT} & 78.7 & 304M & 2020 \\
    DeiT-small~\citep{TouvronCDMSJ21}  & 79.9   & 22M  & 2020 \\
    Inception-ResNet v2~\citep{SzegedyIVA17} & 80.4 & 56M & 2016 \\
    ConvNext-tiny~\citep{convnext22} & 82.5 & 29M & 2022 \\
    PNASNet-5 large~\citep{LiuZNSHLFYHM18} & 82.9   & 86M & 2017\\
    EfficientNet B4~\citep{TanL19} & 83.4 & 19M & 2019 \\ \bottomrule
    \end{tabular}
    \vspace{-0.5em}
\end{table}

We examine 19 model architectures in this work that cover a diverse range of accuracies on ImageNet in order to observe the relationship between ImageNet performance and target dataset performance.
In addition to the commonly used CNNs, we also include data-efficient image transformers (DeiT) due to the recent increase in usage of Vision Transformers.
Additional model details are in Table~\ref{tab:imagenet_models}.

\subsection{Hyperparameter Grid}

Hyperparameter tuning is a key part of neural network training, as using suboptimal hyperparameters can lead to suboptimal performance. Furthermore, the correct hyperparameters vary across both models and training data.
To get the best performance out of each model, we train each model on AdamW with a cosine decay learning rate schedule, SGD with a cosine decay learning rate schedule, and SGD with a multi-step decay learning rate schedule.
We also grid search for optimal initial learning rate and weight decay combinations, searching logarithmically between $10^{-1}$ to $10^{-4}$ for SGD learning rate, $10^{-2}$ to $10^{-5}$ for AdamW learning rate, and $10^{-3}$ to $10^{-6}$ as well as $0$ for weight decay.
All models are pretrained on ImageNet and then fine-tuned on the downstream task.
Additional training details for each dataset can be found in Appendix~\ref{app:training_details}. We also run our hyperparameter grid on CIFAR-10 in Appendix~\ref{app:cifar} to verify that we find a strong relationship between ImageNet and CIFAR-10 accuracy as previously reported by \citet{kornblith2019better}.

